PDE-Based Parameterisation Techniques for Planar Multipatch Domains

This paper presents a PDE-based parameterisation framework for addressing the planar surface-to-volume (StV) problem of finding a valid description of the domain's interior given no more than a spline-based description of its boundary contours. The framework is geared towards isogeometric analysis (IGA) applications wherein the physical domain is comprised of more than four sides, hence requiring more than one patch. We adopt the concept of harmonic maps and propose several PDE-based problem formulations capable of finding a valid map between a convex parametric multipatch domain and the piecewise-smooth physical domain with an equal number of sides. In line with the isoparametric paradigm of IGA, we treat the StV problem using techniques that are characteristic for the analysis step. As such, this study proposes several IGA-based numerical algorithms for the problem's governing equations that can be effortlessly integrated into a well-developed IGA software suite. We augment the framework with mechanisms that enable controlling the parametric properties of the outcome. Parametric control is accomplished by, among other techniques, the introduction of a curvilinear coordinate system in the convex parametric domain that, depending on the application, builds desired features into the computed harmonic map, such as homogeneous cell sizes or boundary layers.

==> sec-basic_scheme.tex <==
\section{A Basic Scheme Based on a Posteriori Refinement}
\label{sect:Adaptive_Basic_Scheme}
One of the main challenges of PDE-based parameterization is selecting an appropriate finite-dimensional spline space $\mathcal{V}_h$. For this, we employ the technique of \textit{Dual Weighted Residual}, which will be the topic of Section \ref{subsect:Adaptive_DWR}.
%%
\subsection{Dual Weighted Residual}
\label{subsect:Adaptive_DWR}
\textit{Dual Weighted Residual}, is an a posteriori error estimation technique that is based on duality considerations. Consider a semi-linear differential form $A(u, \phi)$ (which is linear in $\phi$). We consider the problem
\begin{align}
    \label{eq:Adaptive_DWR_main}
    \text{find } u \in \mathcal{V}^\circ \quad \text{s.t.} \quad A(u, \phi) = f(\phi), \quad \forall \phi \in \mathcal{V}^\circ,
\end{align}
for some linear functional $f(\cdot)$ and a suitably-chosen vector space $\mathcal{V}$, with $\mathcal{V}^\circ = \mathcal{V} \cap H^1_0(\hat{\Omega})$. We seek an approximate solution $u_h \in \mathcal{V}_h^\circ$ with $\mathcal{V}_h \subset \mathcal{V}$ by solving a discretized counterpart of (\ref{eq:Adaptive_DWR_main})
\begin{align}
\label{eq:Adaptive_DWR_main_discretized}
    \text{find } u_h \in \mathcal{V}_h^\circ \quad \text{s.t.} \quad A(u_h, \phi_h) = f(\phi_h), \quad \forall \phi_h \in \mathcal{V}_h^\circ.
\end{align}
Let $L(u)$ be such that
\begin{align}
\label{eq:Adaptive_DWR_DeltaL}
    \Delta L(u_h) \equiv L(u) - L(u_h)
\end{align}
is a quantity of interest (which for instance measures the global quality of the approximation). Furthermore, let
\begin{align}
    \rho(u, \psi) = f(\psi) - A(u, \psi)
\end{align}
denote the residual. \\
If $z$ is the solution of
\begin{align}
    \text{find } z \in \mathcal{V}^\circ \quad \text{s.t.} \quad A^\prime(u, \phi, z) = L^\prime(u, \phi), \quad \forall \phi \in \mathcal{V}^\circ,
\end{align}
we have
\begin{align}
    \Delta L(u_h) = \rho(u_h, z - \psi_h) + R_h(e),
\end{align}
for arbitrary $\psi_h \in \mathcal{V}_h^\circ$ and some $R_h$ that is quadratic in $e \equiv u - u_h$ \cite{rannacher2004adaptive}. In practice, we neglect $R_h$ and approximate $z$ by the solution of the discrete adjoint equation
\begin{align}
\label{eq:Adaptive_DWR_discrete_adjoint}
    \text{find } z_h \in \overline{\mathcal{V}}_h^\circ \quad \text{s.t.} \quad A^{\prime}(u_h, \sigma_h, z_h) = L^{\prime}(u_h, \sigma_h), \quad \forall \sigma_h \in \overline{\mathcal{V}}_h^\circ,
\end{align}
for some adjoint (THB-)spline space $\overline{\mathcal{V}}_h \subset \mathcal{V}$. Hence,
\begin{align}
\label{eq:Adaptive_adjoint_equation_discrete}
    \Delta L(u_h) \simeq \rho(u_h, z_h - \psi_h) = \sum_{w_i \in \left[\mathcal{V}_h \right]} \rho(u_h, w_i(z_h - \psi_h)) \equiv \sum_i \mathbf{r}_i(u_h),
\end{align}
thanks to semi-linearity of $A(\cdot, \cdot)$ and the partition of unity property associated with $\left[ \mathcal{V}_h \right]$. \\
The motivation to use an adjoint spline space that differs from $\mathcal{V}_h$ is the fact that substituting any $z_h \in \mathcal{V}_h^\circ$ in (\ref{eq:Adaptive_adjoint_equation_discrete}) results in $\Delta L(u_h) = 0$ due to Galerkin orthogonality, making it a meaningless error estimate. \\
The appeal of using (\ref{eq:Adaptive_adjoint_equation_discrete}) is that a scalar quantity of interest $\Delta L(u_h)$ is transformed into an integral quantity over $\hat{\Omega}$, which in turn is decomposed into the basis function wise contributions $\mathbf{r}_i(u_h)$. The vector $\mathbf{r}(u_h)$ may then be utilized in the selection of basis functions for goal-oriented refinement (see Section \ref{subsect:Adaptive_Refinement_Strategies}).
\begin{remark}
If $u_h$ is a very inaccurate approximation of $u$, the discrete adjoint solution $z_h$ will be inaccurate regardless of the choice of $\overline{\mathcal{V}}_h$. Heuristically, we have rarely encountered this situation in the examples considered in this work. In case refinement is ineffective, the procedure should be restarted with a uniformly refined initial basis.
\end{remark}

%%

\subsection{Applications to PDE-Based Parameterization}
In this section, we apply the methodology from Section \ref{subsect:Adaptive_DWR} to the PDE-based parameterization problem (\ref{eq:Adaptive_inverse_mapping_approach_PDE_scaled_discretized}). Let $\mathbf{x}_D$ be the canonical extension of the Dirichlet data as introduced in (\ref{eq:Adaptive_inverse_mapping_approach_PDE_scaled_discretized}). With $\mathbf{x}_h = \mathbf{x}_D + \mathbf{x}_0$, we may write (\ref{eq:Adaptive_inverse_mapping_approach_PDE_scaled_discretized}) in the equivalent form
\begin{align}
\label{eq:Adaptive_EGG_problem_DWR_form}
    \text{find } \mathbf{x}_0 \in \mathcal{U}_h^{\mathbf{0}} \quad \text{s.t.} \quad F(\mathbf{x}_D + \mathbf{x}_0, \boldsymbol{\sigma}_h) = 0, \quad \forall \boldsymbol{\sigma}_h \in \mathcal{U}_h^{\mathbf{0}}.
\end{align}
In the formalism of (\ref{eq:Adaptive_DWR_main_discretized}), we hence have $A(\mathbf{x}, \boldsymbol{\sigma}) = F(\mathbf{x}_D + \mathbf{x}, \boldsymbol{\sigma})$ and $f(\boldsymbol{\sigma}) = 0$. Alternatively, we may absorb the dependence on $\mathbf{x}_D$ in $f(\cdot)$. As before, the relation between $\mathcal{V}_h$ and $\mathcal{U}_h^{\mathbf{f}}$ follows from (\ref{eq:THB_basis_main_discrete}). \\
We would like to design scalar cost functions ($L(u)$ in (\ref{eq:Adaptive_DWR_DeltaL})) to aid us in refining an a priori chosen basis $[\mathcal{V}_h]$ such that after recomputing the solution over the refined space $\mathcal{V}_h^R \supset \mathcal{V}_h$,
\begin{enumerate}
    \item $\mathbf{x}_h^R$ is bijective;
    \item $\mathbf{x}_h^R$ approximates $\mathbf{x}$ well.
\end{enumerate}
In a discrete setting, we may relax the condition that $\mathbf{x}_h^R$ be bijective by the condition that $\mathbf{x}_h^R$ has a positive Jacobian determinant in all quadrature points $\Xi = \{\boldsymbol{\xi}_1^q, \ldots, \boldsymbol{\xi}_M^q \}$. \\
As such, let $\mathbf{x}_h$ be the solution of (\ref{eq:Adaptive_EGG_problem_DWR_form}) over the space $\mathcal{V}_h$ and let 
\begin{align}
\label{eq:Adaptive_DWR_quadrature_subset}
    \Xi_{\mathbf{-}} = \left \{ \boldsymbol{\xi}_i^q \in \Xi \enskip \vert \enskip \det J(\mathbf{x}_{h}) < 0 \text{ in } \boldsymbol{\xi}_i^q \right \}.
\end{align}
To address (potential) lack of bijectivity, we propose the following goal-oriented cost function:
\begin{align}
\label{eq:Adaptive_bijectivity_costfunc}
    L_{\Xi}(\mathbf{x}) = \sum_{\boldsymbol{\xi}_i^q \in \Xi_{\mathbf{-}}} \det J(\mathbf{x})(\boldsymbol{\xi}_i^q),
\end{align}
such that
\begin{align}
    \Delta L_{\Xi}(\mathbf{x}_h) = \underbrace{L_\Xi(\mathbf{x})}_{\geq 0} - \underbrace{L_\Xi(\mathbf{x}_h)}_{\leq 0} \geq 0,
\end{align}
with equality if and only if $\Xi_{\mathbf{-}} = \emptyset$. Here, the inequality $L_\Xi(\mathbf{x}) \geq 0$ follows from the Rad\'o-Kneser-Choquet theorem (see Section \ref{sect:Adaptive_Introduction}) while $L_\Xi(\mathbf{x}_h) \leq 0$ follows from (\ref{eq:Adaptive_DWR_quadrature_subset}). According to (\ref{eq:Adaptive_adjoint_equation_discrete}), we may approximate
\begin{align}
\label{eq:Adaptive_DWR_basis_function_split}
    \Delta L_\Xi(\mathbf{x}_h) & \simeq -F(\mathbf{x}_h, \mathbf{z}_h - \boldsymbol{\psi}_h)
                                   = \sum_{w_i \in \left[ \mathcal{V}_h \right]} - F \left(\mathbf{x}_h, w_i( \mathbf{z}_h - \boldsymbol{\psi}_h ) \right) \equiv \sum_i \mathbf{r}_i(\mathbf{x}_h).
\end{align}
Typically, we choose $\boldsymbol{\psi}_h$ as the $L_2(\hat{\Omega}, \mathbb{R}^2)$-projection of $\mathbf{z}_h$ onto $\mathcal{U}_h^{\mathbf{0}}$.
\begin{remark}
Even though subtracting a nonzero $\boldsymbol{\psi}_h \in \mathcal{U}_h^{\mathbf{0}}$ does not alter the outcome on the right hand side of (\ref{eq:Adaptive_DWR_basis_function_split}), it does influence its decomposition into the basis function wise contributions $\mathbf{r}_i(\mathbf{x}_h)$. Here, the proposed choice of $\boldsymbol{\psi}_h$ serves to retain the sharpness of the error bound.
\end{remark}
\noindent Using the basis function wise decomposition of the quantity of interest $\Delta L_\Xi(\mathbf{x}_h)$, the procedure selects a subset of the $w_i \in \left[ \mathcal{V}_h \right]$ and marks them for refinement. We propose selection criteria in Section \ref{subsect:Adaptive_Refinement_Strategies}. \\
After refinement of $\mathcal{V}_h$, we recompute the mapping from the enriched basis $\mathcal{V}_h^R$ and if necessary repeat above steps until discrete bijectivity (over $\Xi$) has been achieved.
\begin{remark}
For better performance, we always use the prolonged coarse-grid solution as an initial guess for recomputing the mapping under the refined basis.
\end{remark}
\noindent Upon completion, we may choose to settle for the (possibly inaccurate but with respect to the $\boldsymbol{\xi}_i^q \in \Xi$ analysis-suitable) resulting mapping $\mathbf{x}_h^R$, or we may choose to further improve its accuracy with respect to the exact solution. As the exact solution of the PDE problem is equal to the minimizer of the Winslow function (see Section \ref{sect:Adaptive_related_work})
\begin{align*}
    L_W(\mathbf{x}) = \int_{\hat{\Omega}} \frac{g_{11} + g_{22}}{ \det J} \mathrm{d} S,
\end{align*}
by choosing $- L_W(\mathbf{x})$ as a cost function, we acquire the quantity of interest
\begin{align}
\label{eq:Adaptive_dWinslow_costfunc}
    \Delta L_W(\mathbf{x}_h) = -L_W(\mathbf{x}) + L_W(\mathbf{x}_h) \geq 0,
\end{align}
with equality for $\| \mathbf{x} - \mathbf{x}_h \|_{H^1(\hat{\Omega})} = 0$. As such, (\ref{eq:Adaptive_dWinslow_costfunc}) may serve as a measure for the distance of $\mathbf{x}_h$ to $\mathbf{x}$. As before, we approximate (\ref{eq:Adaptive_dWinslow_costfunc}) by substituting the discrete adjoint solution $\mathbf{z}_h$ in (\ref{eq:Adaptive_adjoint_equation_discrete}) and base refinement criteria on the basis function wise contributions to (\ref{eq:Adaptive_dWinslow_costfunc}). The steps of refinement, recomputation and adjoint estimation may be repeated until the estimate $\vert \Delta L_W(\mathbf{x}_h) \vert \simeq \vert -F(\mathbf{x}_h, \mathbf{z}_h - \boldsymbol{\psi}_h) \vert$ is deemed sufficiently small. \\
The above methodology is compatible with the direct approach from Section \ref{subsect:Adaptive_Direct_Minimization}. A typical workflow consists of computing a bijection $\mathbf{x}_h$ under the cost function (\ref{eq:Adaptive_bijectivity_costfunc}) using the PDE-based approach and continuing to improve parametric quality using (\ref{eq:Adaptive_dWinslow_costfunc}). Furthermore, once a bijective $\mathbf{x}_h$ has been found, it may serve as an initial guess for the direct approach from Section \ref{subsect:Adaptive_Direct_Minimization}.

%%
\subsection{Choice of Adjoint Basis}
\label{subsect:Adaptive_Adjoint_Basis}
Problem (\ref{eq:Adaptive_DWR_discrete_adjoint}) requires choosing a suitable dual spline space $\mathcal{V} \supset \boldsymbol{\overline{\mathcal{V}}}_h \neq \mathcal{V}_h$, which typically results from uniformly refining $\mathcal{V}_h$ (in either $h$ or the polynomial degree $p$), leading to a $\sim 4$-fold increase in the number of DOFs associated with the (linear) discrete adjoint equation. In a THB-setting, we have the luxury of choosing $\overline{\mathcal{V}}_h$ reminiscent of the role of $K$-refinement \cite{hughes2005isogeometric} in a structured spline setting. Let $(p, \alpha)$ be the degree and regularity of $\mathcal{V}_h$ (which we assume to be equal in both directions for convenience) and let $\mathcal{T}$ denote the corresponding decomposition of $\hat{\Omega}$ into elements. We define $\overline{\mathcal{V}}_K(\mathcal{V}_h)$ as the richest (dimensionality-wise) THB space of degree $p+1$ and regularity $\alpha + 1$ that is compatible with the elements in $\mathcal{T}$. Typically, we have $\operatorname{dim} \overline{\mathcal{V}}_K(\mathcal{V}_h) \simeq \operatorname{dim} \mathcal{V}_h$. \\
While taking $\overline{\mathcal{V}}_h = \mathcal{V}_{h/2}$ yields more accurate adjoint solutions $\mathbf{z}_h \in (\overline{\mathcal{V}}_h^\circ)^2$, we have found the choice $\boldsymbol{\overline{\mathcal{V}}}_h = \overline{\mathcal{V}}_K(\mathcal{V}_h)$, to be sufficient for refinement based on both (\ref{eq:Adaptive_DWR_quadrature_subset}) and (\ref{eq:Adaptive_dWinslow_costfunc}). As such, solving the discrete adjoint equation becomes a cheap operation.

%%
\subsection{Refinement Strategies}
\label{subsect:Adaptive_Refinement_Strategies}
The decomposition into basis function wise contributions $\mathbf{r}_i(\mathbf{x}_h)$ introduced in (\ref{eq:Adaptive_adjoint_equation_discrete}) is particularly useful in a THB-setting since elementwise refinement may not change the dimension of the underlying THB spline space. In the following, we present several strategies for using $\mathbf{r}(\mathbf{x}_h)$ to mark basis functions $w_i \in \left[ \mathcal{V}_h \right]$ for refinement. We define the vectors $\mathbf{w}$ and $\mathbf{\tilde{r}}$ with
\begin{align}
\label{eq:Adaptive_weighted_residual}
    \mathbf{w}_i = \int_{\hat{\Omega}} w_i \mathrm{d} S \quad \text{and} \quad \mathbf{\tilde{r}}_i = \frac{\mathbf{r}_i}{\mathbf{w}_i}.
\end{align}
Furthermore, we let $\mathbf{\tilde{r}}_\text{max} = \max_i |\mathbf{\tilde{r}}_i|$ and $\mathcal{I} = \{1, \ldots, \vert \mathcal{V}_h \vert \}$. Inspired by \cite{prudhomme2003computable}, we define
\begin{align}
\label{eq:Adaptive_Absolute_Maximum_Threshold}
    \mathcal{I}^\alpha_\text{max} = \{ i \in \mathcal{I} \enskip \vert \enskip | \mathbf{\tilde{r}}_i | \geq \beta \mathbf{\tilde{r}}_\text{max} \}
\end{align}
as the index-set of absolutely weighted contributions that exceed the value $\beta \mathbf{\tilde{r}}_\text{max}$, for some $\beta \in [0, 1]$. The $i \in \mathcal{I}^\alpha_\text{max}$ then constitute the indices corresponding to basis functions whose supporting elements $\mathcal{E}^k \in \mathcal{T}$, from the $k$-th level in the element hierarchy, are replaced by finer counterparts $\mathcal{E}^{k+1}$ from the $(k+1)$-th level. Note that the function may, due to preceding refinements of other functions, be already partially supported by $\mathcal{E}^{l} \in \mathcal{T}$, with $l \geq k + 1$. In this case only the coarsest supporting elements $\mathcal{E}^k$ are refined. As a result, upon constructing the canonical THB-spline space over the refined $\mathcal{T}$, $w_i \in \left[ \mathcal{V}_h \right]$ is replaced by several functions from the next level in the hierarchy, leading to a local increase of the DOFs. Basis function wise refinement ensures that always at least one function is removed from the basis and replaced by several finer ones. Naturally, hierarchical refinement based on THB-splines is a somewhat more involved process than this manuscript suggests. For more details, we refer to \cite{giannelli2012thb, van2020adaptive}. \\
Since both (\ref{eq:Adaptive_bijectivity_costfunc}) and (\ref{eq:Adaptive_dWinslow_costfunc}) are strictly positive quantities of interest, disregarding negative contributions in (\ref{eq:Adaptive_weighted_residual}) is a plausible strategy, too. Heuristically, this strategy mildly reduces the total number of required DOFs until bijectivity is achieved. However, this comes at the expense of a larger number of the required a posteriori refinements, which are limited to typically no more than $3-4$ using (\ref{eq:Adaptive_Absolute_Maximum_Threshold}).

\subsection{Results}
\label{subsect:Adaptive_Results}
To demonstrate the appeal of local refinement made possible by THB splines, in the following, we present parameterizations for the U.S. state of Indiana, the German province of North Rhine-Westphalia and the country of Austria, all of which have complicated boundaries but relatively simple interior. The initial basis $\left[ \mathcal{V}_h \right]$ results from refining an initial grid comprised of $7 \times 7$ elements by the boundaries until the contours of $\Omega$ are approximated sufficiently well. In all cases, $\mathcal{V}_h$ is a bicubic hierarchical space. We take $\overline{\mathcal{V}}_h = \overline{\mathcal{V}}_K(\mathcal{V}_h)$ (see Section \ref{subsect:Adaptive_Adjoint_Basis}) and base refinement on (\ref{eq:Adaptive_Absolute_Maximum_Threshold}) with $\beta = 0.2$. The numerical scheme has been implemented in the open-source finite element library \textit{Nutils} \cite{gertjan_van_zwieten_2020_4071707}.

\begin{figure}[h!]
  \centering
  \subfloat{\includegraphics[valign=c, width=0.4 \linewidth]{img/chapter3/domain_final_Indiana.png}}\label{fig:Indiana_domain} $\quad$
  \centering
  \subfloat{\includegraphics[align=c, width=0.55 \linewidth]{img/chapter3/Indiana_alpha02_ndof_2338_fully_optimized.png}\label{fig:Indiana_final}}
  \caption{The domain with canonical bicubic basis of $2338$ DOFs (left) and the THB-spline parameterization of the U.S. state of Indiana (right).}
  \label{fig:Indiana}
\end{figure}

\begin{figure}[h!]
  \centering
  \subfloat{\includegraphics[align=c, width=0.3 \linewidth]{img/chapter3/Domain_Final.png}}\label{fig:NRW_domain} $\qquad$
  \centering
  \subfloat{\includegraphics[align=c, width=0.55 \linewidth]{img/chapter3/NRW_Final.png}\label{fig:NRW_final}}
  \caption{The domain with bicubic basis of $2676$ DOFs (left) and the THB-spline parameterization of the German province of North Rhine-Westphalia (right).}
  \label{fig:NRW}
\end{figure}

\begin{figure}[h!]
  \centering
  \subfloat{\includegraphics[align=c, width=0.27 \linewidth]{img/chapter3/domain_final_Austria_10634.png}}\label{fig:Austria_domain}
  \centering
  \subfloat{\includegraphics[align=c, width=0.72 \linewidth]{img/chapter3/Austria_fully_optimized_ndofs_10634.png}\label{fig:Austria_final}}
  \caption{The domain with bicubic basis comprised of $9640$ DOFs (left) and the THB-spline parameterization of Austria (right).}
  \label{fig:Austria}
\end{figure}

\noindent Figures (\ref{fig:Indiana}) to (\ref{fig:Austria}) clearly demonstrate the DOF savings made possible by local refinement. Not surprisingly, refinement especially affects the protruded and concave areas close to the boundaries. \\
At every refinement level, parameterizations were computed using the Newton-Krylov approach from Section \ref{subsect:Adaptive_Newton}. They were post-processed with the direct approach from Section \ref{subsect:Adaptive_Direct_Minimization} once bijectivity had been achieved. \\
The iterative solver typically converges after $4-5$ nonlinear iterations on the coarsest level plus another $2-3$ iterations per a posteriori refinement. Once bijectivity is achieved, initializing the direct approach from (\ref{eq:Adaptive_Winslow_PDE_discretized}) with the PDE solution typically leads to convergence after fewer than $3$ iterations.

==> sec-control_mechanisms_backup.tex <==
\section{Control Mechanisms}
\label{sect:control_mechanisms}

\subsection{Techniques for Parametric Control}
The parameterisations generated by Winslow's original approach~\eqref{eq:Winslow_pullback} or its PDE-based counterparts perform well on a wide range of benchmark problems \cite{gravesen2012planar}. However, as individual applications may require parameterisations with specific features, such as boundary layers in flow problems or homogeneous cell-sizes in problems subject to a CFL-condition, the techniques from Section \ref{sect:numerical_schemes} may be too rigid. Clearly, choosing the multipatch covering $\mathcal{Q}$ based on the application's specific needs may provide relief. However, in practice, this may prove too restrictive since the covering remains bilinear, which does not, for instance, allow for the creation of boundary layers. \\
Parametric control can be achieved in two main ways:
\begin{enumerate}
    \item Augmenting the standard inverse Laplace problem with a nonhomogeneous diffusivity.
    \item Mapping inversely harmonically into a parametric domain with a curvilinear rather than a Cartesian coordinate system.
\end{enumerate}
Let $\boldsymbol{\phi}: \Om_1 \rightarrow \mathbb{R}^2$ satisfy:
\begin{align}
\label{eq:classical_inverse_laplace_diffusivity}
    i \in \{1, 2\}: \quad \nabla \cdot \left( D \nabla \boldsymbol{\phi}_i \right) = 0 \quad \text{in } \Om_1, \quad \text{s.t. } \boldsymbol{\phi} = \mathbf{F} \text{ on } \partial \Om_1.
\end{align}
For point 1., we state the following theorem \cite{bauman2001univalent}:
\begin{theorem}[Divergence-form equations]
\label{thrm:nondegeneracy_div_form_equations}
   Let $D \in \text{SPD}^{2 \times 2}(\Om_1)$ be uniformly elliptic and let $\boldsymbol{\phi} \in H^1(\Om_1, \mathbb{R}^{2}) \cap C^0(\Om_1, \mathbb{R}^2)$ be the weak solution of~\eqref{eq:classical_inverse_laplace_diffusivity}. If $\mathbf{F}$ is diffeomorphic between $\partial \Om_1$ and $\partial \Om_2$ and $\Om_2$ is convex, then $\boldsymbol{\phi}: \Om_1 \rightarrow \Om_2$ satisfies $\det \partial_{\bx} \boldsymbol{\phi} \geq 0$ a.e. in $\Om_1$.
\end{theorem}
Under stronger regularity requirements on $D$, $\Om_1$ and $\Om_2$, Theorem \ref{thrm:nondegeneracy_div_form_equations} can be extended to uniform nondegeneracy $\det \partial_{\bx} \boldsymbol{\phi} > 0$ (a.e. in $\Om_1$). For details we refer to \cite{bauman2001univalent}. This means in particular that for merely essentially bounded $D \in \text{SPD}^{2 \times 2}(\Om)$, we need to account for the possibility of $\det \partial_{\bxi} \bx \rightarrow 0$ or $\det \partial_{\bxi} \bx \rightarrow \infty$ in the interior of $\hOm$, which may require stabilisation. Taking $\Om_1 = \Om$ and $\Om_2 = \hOm$, it is reasonable to assume that Theorem \ref{thrm:nondegeneracy_div_form_equations} also applies to, for instance, the weak-form approach from Section \ref{subsect:weak_form_discretisation}, even though it exchanges the dependencies, i.e.,  $\bxi(\bx) \rightarrow \bx(\bxi)$. A limitation of introducing a nonhomogeneous diffusivity is that it is currently unknown whether the inverted problem can be cast into a form that does not contain the Jacobian determinant in the denominator, as in the NDF-discretisation from Section \ref{subsect:NDF_discretisations}. However, the NDF-discretisations remain highly practical since they can compute a nondegenerate reference solution to initialise an iterative scheme with $D \neq \mathcal{I}^{2 \times 2}$ based on the weak-form discretisation. \\

\noindent For point 2., a coordinate transformation is conveniently accomplished by introducing a controlmap $\br: \hOm \rightarrow \hOmr$. As such, we now allow the target domain of $\bx^{-1}: \Om \rightarrow \hOmr$ to be a parametric surface, too. In what follows, differential operators receive a subscript to indicate differentiation w.r.t. various coordinate systems. For instance, $\nabla \rightarrow \nabla_{\br}$ to indicate differentiation w.r.t. the entries of $\br: \hOm \rightarrow \hOmr$. \\
The introduction of $\br: \hOm \rightarrow \hOmr$ furthermore enables creating boundary correspondences $\mathbf{F}^{\br \rightarrow \bx}: \partial \hOmr \rightarrow \partial \Om$ that are diffeomorphic between $\hOmr$ and $\Om$ when $\Om$ has no corners by, for instance, choosing $\hOmr$ to be the unit disc. For Theorem \ref{thrm:RKC} to apply to the pair $(\hOmr, \Om)$, we require $\hOmr$ to be convex. We denote the map that maps inversely harmonically into the domain $\Om^{\br} = \br(\hOm)$ by $\bx^{\br}(\br): \hOmr \rightarrow \Om$. The same map can be converted to the original coordinate system via a pullback. We employ the abuse of notation $\bx^{\br}(\br)$ instead of $\bx(\br(\bxi))$ to indicate a change of coordinate system and assume that the reader is aware of the compositions involved. \\
\pichskip{15pt}% Horizontal gap between picture and text
\parpic[r][b]{%
  \begin{minipage}{100mm}
  \centering
    \includegraphics[width=1 \textwidth]{img/control/cover.png}%
    \captionof{figure}{Figure summarising the dependencies between $\bx, \bs, \br, \bxi$ and $\bmu$.}
    \label{fig:dependency_summary}
  \end{minipage}
}

%Given a reference map $\br: \hOm \rightarrow \Om^{\br}$, the purpose of this section is to provide techniques for computing a controlmap $\bs: \hOmr \rightarrow \hOmr$ that introduces a new coordinate system in $\hOmr$ thereby building application-specific features into the map $\bx^{\bs}(\bxi): \hOm \rightarrow \Om$. Here, we distinguish between \textit{a priori} and \textit{a posteriori} techniques, where the former computes $\bs: \hOmr \rightarrow \Om^{\br}$ using only information provided by the reference controlmap $\br: \hOm \rightarrow \hOmr$, while the latter also uses information of the reference solution $\bx^{\br}: \hOmr \rightarrow \Om$. 
%If the recomputed controlmap $\bs(\br): \hOmr \rightarrow \hOmr$ restricted to $\partial \hOmr$ is the identity (i.e., the problem's boundary condition is unchanged), an intuitive interpretation follows from the observation that the continuous problem's solution in $\hOmr$ is given by the composition $\bx^{\bs}(\br) = \bx^{\br} \circ \bs$ \cite{hinz2020goal}. \\

\noindent In the IGA-setting, parametric control via $\br: \hOm \rightarrow \hOmr$ is conveniently achieved by reinterpreting the PDE-based formulations over the Cartesian coordinate system $\bxi = (\xi_1, \xi_2)^T$ as problems posed over $\hat{\Om}^{\br}$, with the curvilinear coordinate system induced by $\br(\bxi) = (r_1(\xi_1, \xi_2), r_2(\xi_1, \xi_2))^T$. We may then use basic differential geometry identities to express the associated integrals in the original coordinate system via a pullback. As such, the operators from Section \ref{sect:numerical_schemes} now receive an additional $\br$-dependence. However, this does not change the nature of the equations as long as the $\br \circ \bm^i$ remain diffeomorphisms. \\

As in point 1., a broad class of reparameterisation methods follows from seeking the controlmap as the solution of~\eqref{eq:classical_inverse_laplace_diffusivity}. More precisely, given a reference controlmap $\br: \hOm \rightarrow \hOmr$, we may find a new controlmap $\bs(\br): \hOmr \rightarrow \hOmr$ by solving~\eqref{eq:classical_inverse_laplace_diffusivity} with $\Om_1 = \Om_2 = \hOmr$ while selecting a diffusivity $D$ that builds desired features into the solution. The map $\bs(\bxi): \hOm \rightarrow \Om^{\br}$ then follows from a pullback and a diffeomorphic boundary correspondence $\mathbf{F}^{\br \rightarrow \bs}: \partial \hOmr \rightarrow \hOmr$ is given by the identity.
% $\bx^{\bs}(\bxi): \hOm \rightarrow \Om$ after recomputation under $\bs(\bxi): \hOm \rightarrow \Om^{\br}$. The most convenient formulation seeks a controlmap $\bs(\br): \hOmr \rightarrow \hOmr$ as the solution of~\eqref{eq:classical_inverse_laplace_diffusivity} posed over $\Om^{\br}$. A diffeomorphic boundary correspondence $\mathbf{F}^{\br \rightarrow \bs}$ is given by the identity while $\bs(\bxi): \hOm \rightarrow \hOmr$ follows from a pullback. 
\noindent If $\bs(\br): \hOmr \rightarrow \hOmr$ is the identity on $\partial \hOmr$, the effect of the coordinate transformation, induced by $\bs(\bxi): \hOm \rightarrow \hOmr$, on $\bx^{\bs}(\bxi): \hOm \rightarrow \Om$ can be predicted by noting that $\bx^{\bs}(\bxi) = \bx^{\br} \circ \bs(\bxi)$. All the dependencies between $\bx, \bs, \br, \bxi$ and the local coordinate system $\bmu$ in $\Omega^{\square}$ are summarised in Figure \ref{fig:dependency_summary}. \\

\noindent As before, depending on the regularity of the diffusivity, the solutions may contain singularities $\det J \rightarrow 0$ or unbounded growth, i.e., $\det J \rightarrow \infty$. While the vanishing or diverging of $\det J$ is typically avoided by discrete approximations, this behaviour will be observable in a refinement study. For the $\bs(\bxi) \circ \bm^i$ to be diffeomorphisms, this means that for $\bs \in H^1(\hOmr, \mathbb{R}^{2})$, jumps in the Jacobian $\partial_{\br} \bs(\br)$ may only occur on the $\br(\partial \hOm_i)$. As such, we require the diffusivity to be patchwise continuous. \\

\noindent Given a reference controlmap $\br: \hOm \rightarrow \hOmr$, the most general approach combines methods $1.$ and $2.$, leading to the coupled system
\begin{align}
\label{eq:domain_optimisation_coupled_equation}
   \text{find } (\bx(\br), \bs(\br)) \quad \text{ s.t. for } i \in \{1, 2 \}: \left \{ \begin{array}{c} \nabla_{\bx} \cdot \left(D^{\bx} \nabla_{\bx} \bs_i \right) = 0 \\ \nabla_{\br} \cdot \left(D^{\bs} \nabla_{\br} \bs_i \right) = 0 \end{array} \right. \text{ in } \hOmr \quad \text{ and } \quad \left \{ \begin{array}{l} \bx = \mathbf{F}^{\br \rightarrow \bx} \\ \bs = \mathbf{F}^{\br \rightarrow \bs} \end{array} \right. \text{ on } \partial \hOmr,
\end{align}
where, typically, $\mathbf{F}^{\br \rightarrow \bs}(\br) = \br$. Here, the practically useful dependencies are $D^{\bx} = D^{\bx}(\bs, \bx)$ and $D^{\bs} = D^{\bs}(\br, \bx)$. Note that the first equation is inverted and the unknown becomes the differential operator $\nabla_{\bx}$ as a function of $\bx(\br): \hOmr \rightarrow \Om$. The system is associated with a global operator comprised of two separate operators, one for each equation
\begin{align}
\label{eq:domain_optimization_coupled}
    \mathcal{L}^{\bx, \bs}(\bx, \bs, \boldsymbol{\phi}_1, \boldsymbol{\phi}_2, D^{\bx}, D^{\bs}) = \mathcal{L}^{\bx}(\bx, \boldsymbol{\phi}_1, D^{\bx}, \bs) + \mathcal{L}^{\bs}(\bs, \boldsymbol{\phi}_2, D^{\bs}, \bx).
\end{align}
For $D^{\bx} = \mathcal{I}^{2 \times 2}$, the operator $\mathcal{L}^{\bx}(\cdot, \, \cdot, \, \cdot, \, \cdot)$ can be based on any of the operators from Section \ref{sect:numerical_schemes}. For $D^{\mathbf{x}} \neq \mathcal{I}^{2 \times2}$ we restrict ourselves to the weak-form discretisation. With $\bs = \bs(\br)$, the regularised weak-form operator becomes (c.f. equation~\eqref{eq:inverse_elliptic_weak_pullback_operator}):
\begin{align}
\label{eq:weak_form_operator_controlmap}
    \mathcal{L}^{\text{W}}_{\varepsilon}(\bx, \boldsymbol{\phi}, D^{\bx}, \bs) = \int \limits_{\hOmr}\frac{\left(C(\partial_{\br} \bs) \nabla_{\br} \boldsymbol{\phi} \right) \, \colon \left(Q^T(\partial_{\br} \bx, \partial_{\br} \bs) D^{\bx}(\bs, \bx) \, Q(\partial_{\br} \bx, \partial_{\br} \bs) \right)}{\mathcal{R}_{\varepsilon} \left( \det Q(\partial_{\br} \bx, \partial_{\br} \bs) \right)} \, \mathrm{d} \br,
\end{align}
with
$$
Q(\partial_{\br} \bx, \partial_{\br} \bs) := C(\partial_{\br} \bx) \left(\nabla_{\br} \bs \right) \quad \text{and } C(\, \cdot \,) \text{ as in~\eqref{eq:A_CC}.}
$$
The operator corresponding to the second part $\nabla_{\br} \cdot \left(D^{\bs} \nabla_{\br} \bs \right) = 0$ reads
\begin{align}
    \mathcal{L}^{\bs}(\bs, \boldsymbol{\phi}, D^{\bs}, \bx) = \int \limits_{\hOmr} \partial_{\br} \boldsymbol{\phi} \, \colon \, ( \partial_{\br} \bs \, D^{\bs}(\br, \bx)) \, \mathrm{d} \br.
\end{align}
We note that the coordinate transformation $\partial_{\bxi} \rightarrow \partial_{\bs(\bxi)}$ in the NDF operators from Section \ref{subsect:NDF_discretisations} reintroduces the Jacobian determinant $\det \partial_{\bxi} \bs$ in the denominator upon pullback of the equations from $\hOmr$ into $\hOm$. As such, an iterative algorithm has to be initialised with a nondegenerate controlmap $\bs^0: \hOmr \rightarrow \hOmr$ when $\bx^{\bs}: \hOm \rightarrow \Om$ and $\bs: \hOmr \rightarrow \hOmr$ are coupled via $D^{\bx}$ or $D^{\bs}$. In this case, we recommend basing the scheme on~\eqref{eq:weak_form_operator_controlmap} instead. In the classical literature, parametric control via $\bs$, rather than through a pullback, is accomplished by introducing additional terms in~\eqref{eq:EGG_classical} \cite[Chapter~4]{thompson1998handbook}. While this formulation enables removing $\partial_{\bxi} \bs$ from the denominator, it is not applicable if $\bs \notin H^2(\hOm, \mathbb{R}^2)$ since it requires second-order derivative information of $\bs(\bxi)$, making it unsuited for this paper's use-cases. While it may be possible to reduce the regularity requirements of $\bs: \hOmr \rightarrow \hOmr$ in a way anologous to Section \ref{subsect:NDF_discretisations}, this is beyond the scope of this paper.\\

Given a reference controlmap $\br: \hOm \rightarrow \hOmr$, the controlmap $\bs: \hOmr \rightarrow \hOmr$ is conveniently built from a push-forward of the same finite-dimensional space $\mathcal{V}_h$ used to represent the map $\bx_h: \hOm \rightarrow \Om$. As mentioned before, substituting a degenerate intermediate controlmap $\bs: \hOmr \rightarrow \hOmr$, produced by an iterative root-finding algorithm applied to the coupled system, may cause problems due to division by zero. In practice this is avoided by initialising the scheme by the tuple $(\bx^{\br}, \br)$ (i.e., the solution for $D^{\bx} = D^{\bs} = \mathcal{I}^{2 \times 2}$ over the reference controlmap $\br: \hOm \rightarrow \hOmr$) which is computed using one of the NDF-discretisation from Section \ref{subsect:NDF_discretisations}. The barrier term in~\eqref{eq:weak_form_operator_controlmap} then prevents intermediate iterates $(\bx^{\bs}, \bs)^i$ from leaving the set of nondegenerate maps. As before, a discretisation takes the test functions $(\boldsymbol{\phi}_1, \boldsymbol{\phi}_2)$ from the finite-dimensional space $\mathcal{U}_h^{\mathbf{0}} \times \mathcal{U}_h^{\mathbf{0}}$ and finds the root using Newton's method. In practice, the coupled scheme converges reliably for a wide range of diffusivities $D^\bx, D^{\bs}$ when initialised with $(\bx^{\br}, \br)$. \\

\noindent Depending on the choice of $D^{\bx}$ and $D^{\bs}$, the solution of the coupled system may no longer be uniformly nondegenerate (even for boundary correspondences that lead to UNDG maps for $D = \mathcal{I}^{2\times2}$). To avoid singularities, we shall often introduce a stabilisation on the patch vertices. As such, let $\Gamma^v = \{ \mathbf{v}^1, \ldots, \mathbf{v}^{N_v} \} \subset \overline{\hOm}$ be the set of patch vertices shared by at least two patches, i.e.,
$$\Gamma^v := \left \{ \mathbf{v} \in \overline{\hOm} \, \, \big| \, \, \exists (i, j) \in \{1, \ldots, N_p\} \times \{1, \ldots, N_p\} \text{ s.t. } \overline{\hOm}_i \cap \overline{\hOm}_j = \{ \mathbf{v} \} \right \}.$$
The singularities are avoided by introducing an appropriate regularisation. For this purpose, we introduce the Gaussian blending functions
\begin{align}
\label{eq:exponential_decay_regularisation}
    g_i^{\kappa}(\br) := A_i \exp{\left(-\left(\frac{\kappa}{d_i^{\text{min}}} \| \br - \br(\mathbf{v}^i) \| \right)^2 \right)}, \quad \text{with} \quad d_i^{\min} := \min \left \{ \|\mathbf{v}^i - \mathbf{v}^j \| \, \, \big| \, \, j \in \{1, \ldots, N_p\} \setminus \{i\} \right \}
\end{align}
and $\kappa > 0$. Here, the $A_i$ are chosen such that
$$\forall \mathbf{v}^i \in \Gamma^v: \quad \sum_{i=1}^{N_v} g_i^{\kappa}(\br(\mathbf{v}^i)) = 1.$$
Let $D$ be the diffusivity in question and let $\mathcal{D}_i = \{D_i^1, \ldots, D_i^q \}$ be the set containing the limits
$$D_i^j := \lim \limits_{\bxi \rightarrow \mathbf{v}^i} D(\br(\bxi)) \quad \text{ s.t. } \bxi \in \hOm_j \quad \text{for each patch } \hOm_j \text{ with } \overline{\hOm}_j \cap \{\mathbf{v}^i\} = \{ \mathbf{v}^i \}.$$
We define $\overline{D}_i$ as the average of the $D_i^j \in \mathcal{D}_i$, i.e.,
\begin{align}
\label{eq:heuristical_D_scaling}
    \overline{D}_i := \sum \limits_{D_i^j \in \mathcal{D}_i} D_i^j.
\end{align}
The regularisation ensures that the regularised $\overline{D}^{\kappa}(D) \in \text{SPD}^{2 \times 2}(\hOmr)$ is single-valued in the $\br(\mathbf{v}^i)$ by replacing
\begin{align}
\label{eq:patch_vertex_stabilisation}
    D \rightarrow \overline{D}^{\kappa}(D) := \left( 1 - \sum \limits_{i=1}^{N_v} g_i^{\kappa} \right) D + \sum_{i=1}^{N_v} g_i^{\kappa} \overline{D}_i.
\end{align}
The decay rate $\kappa > 0$ in~\eqref{eq:exponential_decay_regularisation} tunes the degree of regularisation and is relatively insensitive to the characteristic length-scale of $\Omega^{\br}$ thanks to the scaling by $d_i^{\min}$. It should be noted that other regularisations exist besides~\eqref{eq:heuristical_D_scaling}.

%\noindent Given some nondegenerate $\bx_h \in \mathcal{U}^{\mathbf{F}}_h$ and a reference controlmap $\br: \hOm \rightarrow \hOmr$, it should be mentioned that the controlmap $\bs(\bxi): \hOm \rightarrow \hOmr$ that would produce $\bx_h(\bxi): \hOm \rightarrow \Om$ under the inverse harmonicity requirement can be approximated by approximately solving the partially integrated variational counterpart of
%\begin{align}
%\label{eq:find_controlmap_given_x}
%\Delta \bs = \mathbf{0} \quad \text{in } \Om, \quad \text{s.t.} \quad \bs = \left( \mathbf{F}^{\br \rightarrow \bx} \right)^{-1} \text{ on } \partial \Om,
%\end{align}
%where $\mathbf{F}^{\br \rightarrow \bx}: \partial \hOmr \rightarrow \partial \Om$ denotes the boundary correspondence between $\partial \hOmr$ and $\partial \Om$. \\
To better see what the effect of reparameterising under a nonhomogenous diffusivity $D$ is, we note that~\eqref{eq:classical_inverse_laplace_diffusivity} is the Euler-Lagrange equation of
%\begin{align}
%\label{eq:laplace_reparam_minimisation}
%    \min \limits_{\bs: \hOmr \rightarrow \Om^{\bs}} \int \limits_{\hOmr} D \, \colon \left(\partial_{\br} \bs_i \otimes \partial_{\br} \bs_i \right) \mathrm{d} \br 
%    \quad \text{s.t.} \quad \bs = \mathbf{F}^{\br \rightarrow \bs} \text{ on } \partial \hOmr,
%\end{align}
\begin{align}
\label{eq:laplace_reparam_minimisation}
    \min \limits_{\boldsymbol{\phi}: \Om_1 \rightarrow \Om_2} \frac{1}{2} \int \limits_{\Om_1} \operatorname{tr} \left(\nabla_{\bx} \boldsymbol{\phi}^T D \nabla_{\bx} \boldsymbol{\phi} \right) \mathrm{d} \bx 
    \quad \text{s.t.} \quad \boldsymbol{\phi} = \mathbf{F} \text{ on } \partial \Om_1.
\end{align}
The interpretation as a minimisation problem is helpful in predicting the effect of $D$ on $\boldsymbol{\phi}: \Om_1 \rightarrow \Om_2$.


\subsection{Patch interface removal}
\label{subsect:interface_removal}
The images of local (in $\Om^{\square}$) isolines under the $\bx^{\br}(\bxi) \circ \bm^i$ will generally form a (possibly steep) angle across patch interfaces when joined together on $\Om$. In certain applications, it may be desirable to decrease or largely remove the steep interface angles. As $\bx: \hOmr \rightarrow \Om$ is diffeomorphic in $\hOmr$, a controlmap $\bs: \hOmr \rightarrow \hOmr$ that removes steep angles will, by extension, remove them in the recomputed map $\bx^{\bs}: \hOm \rightarrow \Om$. As such, interface removal can be regarded as an \textit{a priori} step since it requires no prior knowledge of $\bx: \hOm \rightarrow \Om$. \\
%Clearly, seeking $\bs: \hOm \rightarrow \hOm$ as the solution of~\eqref{eq:laplace_reparam_classical}, implies that on the interfaces $\gamma_{jk} \in \Gamma^I$, the controlmap will satisfy
%\begin{align}
%    \forall (i, \gamma_{jk}) \in \{1, 2 \} \times \Gamma^I: \quad [\![ D \nabla_{\bxi} \bs_i \cdot \mathbf{n} ]\!] = 0  \quad \text{on } \gamma_{jk},
%\end{align}
We would like to accomplish
\begin{align}
\label{eq:local_jump_0}
    \forall \gamma_{jk} \in \Gamma^I: \quad  [\![ (\partial_{\bmu^{\perp}} \bs(\br))]\!] = 0  \quad \text{on } \br(\gamma_{jk}),
\end{align}
wherein $[\![ \, \cdot \, ]\!]$ now denotes the ordinary entry-wise jump term while $\partial_{\bmu^{\perp}}$ denotes the directional derivative transversal to $\br(\gamma_{ij})$ (i.e., either $\partial_{\mu_1}$ or $\partial_{\mu_2}$ on $\br(\gamma_{jk}^+)$ and $\br(\gamma_{jk}^-)$). Requirement~\eqref{eq:local_jump_0} can be weakly enforced by utilising in~\eqref{eq:domain_optimisation_coupled_equation} the diffusivity
\begin{align}
\label{eq:laplace_local_trace_penalty}
    D^{\bs}(\br, \bx) = D^{\bs}_{\Gamma^I}(\br) := \partial_{\mu_1} \br \otimes \partial_{\mu_1} \br + \partial_{\mu_2} \br \otimes \partial_{\mu_2} \br \quad \text{on} \quad \br(\hat{\Omega}_i).
\end{align}
Meanwhile, if $D^{\bx} = \mathcal{I}^{2 \times 2}$,~\eqref{eq:domain_optimisation_coupled_equation} is decoupled and the map $\bx(\bxi): \hOm \rightarrow \Om$ can be computed from a degenerate initial guess using an NDF-discretisation. The diffusivity from~\eqref{eq:laplace_local_trace_penalty} urges $\bs: \hOmr \rightarrow \hOmr$ to map the patchwise isolines $\bs(\bmu)$ smoothly across patch interfaces.
As the magnitude of $\partial_{\mu_i} \br$ depends on $\br \circ \bm^i: \Om^{\square} \rightarrow \br(\hOm_i)$ (and may therefore be subject to considerable changes between patches), the best results are obtained by a normalisation, i.e.,
\begin{align}
\label{eq:laplace_local_normalised_trace_penalty}
    D^{\bs}(\br, \bx) = \widehat{D}^{\bs}_{\Gamma^I}(\br) := \widehat{\partial}_{\mu_1} \br \otimes \widehat{\partial}_{\mu_1} \br + \widehat{\partial}_{\mu_2} \br \otimes \widehat{\partial}_{\mu_2} \br \quad \text{on} \quad \br(\hat{\Omega}_i), \quad \text{with } \widehat{\partial}_{\mu_i} \br := \frac{1}{\left \| \partial_{\boldsymbol{\mu_i}} \br \right \|} \partial_{\boldsymbol{\mu_i}} \br.
\end{align}
Note that 
$$\operatorname{tr}(\mathcal{I}^{2 \times 2}) = \operatorname{tr}\left(\widehat{D}^{\bs}_{\Gamma^I}(\br) \right) = 2.$$
The normalisation has a similar effect as minimising~\eqref{eq:local_jump_0} while now suppressing jumps in the normalised transversal component of the $\br(\gamma_{jk})$ with $\gamma_{jk} \in \Gamma^I$, i.e., we are penalising jumps in the transverse direction but not the direction's magnitudes.
\begin{figure}[h!]
\centering
    \includegraphics[width=0.4 \textwidth]{img/control/interface_removal/benchmark1_param.png} \hspace*{0.5cm}
    \includegraphics[width=0.4 \textwidth]{img/control/interface_removal/benchmark1_geom.png}
\caption{The screw geometry after suppression of local transverse gradient jumps.}
\label{fig:male_screw_interface_remove_k0}
\end{figure}
\noindent We are considering the screw geometry from Figure \ref{fig:male_screw_benchmark_geom} and perform interface removal with normalisation. Figure \ref{fig:male_screw_interface_remove_k0} shows the resulting reparameterisation. As a measure of the degree of interface removal, we utilise the following value
\begin{align}
\label{eq:interface_removal_norm}
    L_{\Gamma}^2(\bx) = \sum \limits_{\gamma_{jk} \in \Gamma^I} \int \limits_{\br(\gamma_{jk})} \left\| [\![ \widehat{\partial}_{\bmu^{\perp}} \bx(\br)]\!] \right \|^2 \mathrm{d} \Gamma,
\end{align}
where $\widehat{\partial}_{\bmu^{\perp}}$ denotes the normalised directional derivative transverse to $\br(\gamma_{jk})$. With
$$\frac{L_{\Gamma}(\bx_h^{\bs})}{L_{\Gamma}(\bx_h)} \approx 0.0998$$ %\quad \text{and} \quad \frac{L_{\text{Area}}(\bx_h^{\bs})}{L_{\text{Area}}(\bx_h)} \approx 1.007,$$
the technique is highly effective. \\ % at suppressing jumps at the expense of a marginal reduction in the cell size homogeneity. \\
As stated in Theorem \ref{thrm:nondegeneracy_div_form_equations}, methods based on~\eqref{eq:domain_optimisation_coupled_equation} do not exclude singularities in $\bs: \hOmr \rightarrow \hOm^{\bs}$. While singularities are in practice avoided by discrete approximations, for merely essentially bounded $D^{\bs} \in \text{SPD}^{2 \times 2}(\hOmr)$, we may expect 
$$\inf \limits_{\hOmr} \det \partial_{\br} \bs \rightarrow 0 \quad \text{or} \quad \sup \limits_{\hOmr} \det \partial_{\br} \bs \rightarrow \infty$$
in a refinement study. For patchwise continuous $D^{\bs} \in \text{SPD}^{2 \times 2}(\hOmr)$, singularities (and unbounded gradients) are exclusively located in the $\br(\mathbf{v}^i)$ with $\mathbf{v}^i \in \Gamma^v$ \emph{[citation forthcoming]}. The creation of singularities can be avoided by employing the stabilisation from~\eqref{eq:patch_vertex_stabilisation}. We are considering the rectangular parametric domain $\hOm = \hOmr$ along with an irregular multipatch covering depicted in Figure \ref{fig:interface_removal_regularised_ref}.
\begin{figure}[h!]
\centering
    \includegraphics[width=0.7 \textwidth, align=c]{img/control/interface_removal/regularised/xi_mu_9.png}
\caption{Bilinear multipatch covering of a rectangular domain comprised of $24$ patches.}
\label{fig:interface_removal_regularised_ref}
\end{figure}
\noindent We perform a refinement study of (normalised) interface removal with and without regularisation, initially assigning a uniform cubic knotvector with three internal knots to each side $L_i \in \Gamma^B$ and facet $\gamma_{ij} \in \Gamma^I$. Each refinement $h \rightarrow h/2$ halves the knotvector's knotspans. We are monitoring the value of $\nu_{\Gamma}( \, \cdot \,) := L_{\Gamma}(\, \cdot \,) / L_{\Gamma}(\br)$ for the original $\bs: \hOmr \rightarrow \hOmr$ and its regularised counterpart $\bs^{\text{reg}}: \hOmr \rightarrow \hOmr$, as well as the values $\min \det J_{\mathbf{v}}(\, \cdot \,)$ and $\max \det J_{\mathbf{v}}(\, \cdot \,)$ which are the minimum and maximum values of $\det \partial_{\br}( \, \cdot \, )$ over all patch vertices $\br(\mathbf{v}^i)$. As $\det \partial_{\br}(\, \cdot \,)$ is not single-valued in the $\mathbf{v}^i \in \Gamma^v$, we define this value as the minimum / maximum of taking the limit on each adjacent patch. Table \ref{tab:refinement_study_regularised_int_removal_mu_inf} contains the reference values in the absence of regularisation while Table \ref{tab:refinement_study_regularised_int_removal_mu_9} contains the corresponding values for the regularisation $D^{\bs} \rightarrow \overline{D}^{\kappa}(D^{\bs})$ with $\kappa = 9$. Furthermore, Figure \ref{fig:interface_removal_regularised} shows the controlmap with and without regularisation after the last refinement level. Table \ref{tab:refinement_study_regularised_int_removal_mu_inf} clearly demonstrates that $\min \det J_{\mathbf{v}}(\, \cdot \,)$ and $\max \det J_{\mathbf{v}}(\, \cdot \,)$ shrink / grow unboundedly in the absence of regularisation while Table \ref{tab:refinement_study_regularised_int_removal_mu_9} demonstrates that regularisation prevents further shrinkage / growth under refinement. 

\begin{table}[h!]
\renewcommand{\arraystretch}{1.5}
\centering
\begin{tabular}{c|c|c|c|c|c}
  & h & h/2 & h/4 & h/8 & h/16 \\
 \hline
$\nu_{\Gamma}(\bs)$ & 0.273 & 0.197 & 0.162 & 0.140 & 0.0991 \\
\hline
$\min \det J_{\mathbf{v}}(\bs)$ & 0.0679 & 0.0466 & 0.0357 & 0.0294 & 0.0184 \\
\hline
$\max \det J_{\mathbf{v}}(\bs)$ & 7.46 & 11.9 & 15.6 & 18.9 & 30.1
\end{tabular}
\caption{Reference values of performing interface removal on the quadrangulation from Figure \ref{fig:interface_removal_regularised_ref} in the absence of regularisation.}
\label{tab:refinement_study_regularised_int_removal_mu_inf}
\end{table}

\begin{table}[h!]
\renewcommand{\arraystretch}{1.5}
\centering
\begin{tabular}{c|c|c|c|c|c}
 $\kappa=9$ & h & h/2 & h/4 & h/8 & h/16 \\
 \hline
$\nu_{\Gamma}(\bs^{\text{reg}})$ & 0.426 & 0.413 & 0.407 & 0.406 & 0.406 \\
\hline
$\min \det J_{\mathbf{v}}(\bs^{\text{reg}})$ & 0.223 & 0.262 & 0.251 & 0.249 & 0.248 \\
\hline
$\max \det J_{\mathbf{v}}(\bs^{\text{reg}})$ & 4.44 & 3.93 & 3.84 & 3.86 & 3.84
\end{tabular}
\caption{The outcomes of performing regularised interface removal with $\kappa = 9$.}
\label{tab:refinement_study_regularised_int_removal_mu_9}
\end{table}

\begin{figure}[h!]
\centering
    \includegraphics[height=3.0cm, align=c]{img/control/interface_removal/regularised/s_mu_9_label.png} \includegraphics[height=3.0cm, align=c]{img/control/interface_removal/regularised/s_mu_9_detJ0_zoom_label.png} \includegraphics[height=3.0cm, align=c]{img/control/interface_removal/regularised/s_mu_9_detJinf_zoom_label.png} \\
    \includegraphics[height=3.0cm, align=c]{img/control/interface_removal/regularised/s_reg_mu_9.png}
    \includegraphics[height=3.0cm, align=c]{img/control/interface_removal/regularised/s_reg_mu_9_detJ0_zoom.png} \includegraphics[height=3.0cm, align=c]{img/control/interface_removal/regularised/s_reg_mu_9_detJinf_zoom.png}
\caption{Plot of the controlmaps $\bs: \hOm \rightarrow \hOm$ (top) and $\bs^{\text{reg}}: \hOm \rightarrow \hOm$ (bottom) along with a zoom-in onto vertices in which the Jacobian determinant grows / shrinks unboundedly in the absence of regularisation.}
\label{fig:interface_removal_regularised}
\end{figure}

\noindent As expected, the regularisation also prevents monotone decrease of $\nu_{\Gamma}(\bs^{\text{reg}})$, eventually settling for a value of $\sim 0.4 L_{\Gamma}(\br)$ relative to the reference value of Figure \ref{fig:interface_removal_regularised_ref}. Meanwhile, the corresponding value shrinks unboundedly in the absence of regularisation. \\
For larger values of $\kappa$, we expect the discretisation to settle for a lower value of $\nu_{\Gamma}(\bs^{\text{reg}})$ at the expense of reducing / increasing the values of $\min \det J_{\mathbf{v}}(\bs^{\text{reg}})$ and $\max \det J_{\mathbf{v}}(\bs^{\text{reg}})$. Table \ref{tab:refinement_study_regularised_int_removal_mu_18} contains the outcomes for regularisation with $\kappa = 18$.

\begin{table}[h!]
\renewcommand{\arraystretch}{1.5}
\centering
\begin{tabular}{c|c|c|c|c|c}
 $\kappa=18$ & h & h/2 & h/4 & h/8 & h/16 \\
 \hline
$\nu_{\Gamma}(\bs^{\text{reg}})$ & 0.315 & 0.314 & 0.309 & 0.303 & 0.299 \\
\hline
$\min \det J_{\mathbf{v}}(\bs^{\text{reg}})$ & 0.0892 & 0.143 & 0.179 & 0.174 & 0.167 \\
\hline
$\max \det J_{\mathbf{v}}(\bs^{\text{reg}})$ & 6.36 & 6.98 & 6.33 & 6.16 & 6.08
\end{tabular}
\caption{The outcomes of performing regularised interface removal with $\kappa = 18$.}
\label{tab:refinement_study_regularised_int_removal_mu_18}
\end{table}
\noindent Indeed, the table confirms this expectation, settling for a value of $\sim 0.3 L_{\Gamma}(\br)$ while roughly doubling the shrinkage / growth of $\det \partial_{\br}(\bs^{\text{reg}})$ compared to $\kappa = 9$. \\
We conclude that the proposed regularisation is an effective means to tune the degree of interface removal at the expense of cell size homogeneity reduction. In practice, an appropriate choice of the decay rate $\kappa > 0$ is furthermore relatively insensitive to the average distance between the $\mathbf{v}^i \in \Gamma^v$, thanks to the scaling by $d_i^{\min}$ in~\eqref{eq:exponential_decay_regularisation}.

\subsection{Cell size homogenisation}
\label{subsubsect:cell_size_hom}
A popular measure for the parameterisation's cell size homogeneity is the \textit{Area} functional
\begin{align}
    L_{\text{Area}}(\bx) = \int \limits_{\hOm} \left(\det J(\bx) \right)^2 \mathrm{d} \bxi,
\end{align}
which measures the variance of $\det J(\bx)$ over $\hOm$, with smaller values indicating better homogeneity. In the multipatch setting, it is more natural to measure the homogeneity on each individual patch and summing over all patches
\begin{align}
\label{eq:Area_multipatch}
    L_{\text{Area}}(\bx) := \sum_{i=1}^{N_p} \int \limits_{\Om^{\square}} \left( \det \partial_{\bmu} (\bx(\bxi) \circ \bm^i) (\bmu) \right)^2 \mathrm{d} \bmu,
\end{align}
wherein $\bmu = (\mu_1, \mu_2)^T$ denotes the free coordinate functions in $\Om^{\square}$. Direct minimisation of~\eqref{eq:Area_multipatch} over the map's inner controlpoints leads to a nonconvex problem which is furthermore prone to yielding degenerate maps. \\
We notice that for $D^{\bx} = \mathcal{I}^{2 \times 2}$, the solution of the inverse Laplace problem is merely a property of the shapes $\hOmr$ and $\Om$ as well as the diffeomorphic boundary correspondence $\mathbf{F}^{\br \rightarrow \bx}: \partial \hOmr \rightarrow \partial \Om$. As such, a controlmap $\bs: \hOmr \rightarrow \hOmr$ that is the identity on $\partial \hOmr$ computes the composition $\bx^{\bs}(\br) = \bx^{\br} \circ \bs(\br)$. Therefore, we may require $\bs(\br)$ to contract cells in $\br(\hOm_i)$ wherever $\det \partial_{\bmu} \bx^{\bs}(\br)$ is large and vice versa. We may also choose to penalise based on $\partial_{\bxi} \bx^{\bs}(\br)$ or $\partial_{\br} \bx^{\bs}(\br)$ to reduce the Area functional in a different coordinate system if desired. \\
To cast this problem into the form of~\eqref{eq:domain_optimization_coupled}, we contract the cells of $\bs(\br)$ by penalising the value of $\operatorname{tr}(G^{\br \rightarrow \bs})$, where $G^{\br \rightarrow \bs}$ denotes the metric between the coordinate systems induced by $\br: \hOm \rightarrow \hOm^{\br}$ and $\bs: \hOm^{\br} \rightarrow \hOm^{\br}$. This is accomplished by introducing $D^{\bs}(\br, \bx^{\bs}) = \sigma(\bx^{\bs}) \mathcal{I}^{2 \times 2}$, where $\sigma(\bx^{\bs})$ assumes large values in regions where contraction is desired and vice-versa. For instance
$$\sigma^k(\bx^{\bs})(\br) = (\det \partial_{\bmu} \bx^{\bs}(\br))^k \quad \text{on} \quad \br(\hOm_i),$$
where larger values of $k > 0$ lead to a more drastic homogenisation. As such, we are solving the coupled system~\eqref{eq:domain_optimization_coupled} with $D^{\bx} = \mathcal{I}^{2 \times 2}$ and 
\begin{align}
\label{eq:cell_size_hom_diffusivity}
    D^{\bs}(\bx^{\bs}) = \sigma^k(\bx^{\bs}) \mathcal{I}^{2 \times 2}.
\end{align}
%For this, we propose the following convex quadratic a posteriori minimisation problem
%\begin{align}
%\label{eq:poisson_area_multipatch}
%    \min \limits_{\bs: \hOmr \rightarrow \hOmr} \sum_{i=1}^{N_p} \int \limits_{\br(\hOm_i)} \left( \det \partial_{\bmu} \bx^{\br} \right)^k \operatorname{tr}\left( G^{\br \rightarrow \bs} \right) \mathrm{d} \br \quad \text{s.t.} \quad \bs = \br \text{ on } \partial \hOmr,
%\end{align}
%wherein $G^{\br \rightarrow \bs} = G^{\br \rightarrow \bs}(\br)$ denotes the controlmap's metric tensor over $\br$ while $\det \partial_{\bmu} \bx = \det \partial_{\bmu} \bx(\br)$ is now regarded as a function over $\hOmr$. The formulation from~\eqref{eq:poisson_area_multipatch} urges the the minimisation to reduce the value of $\operatorname{tr}(G^{\br \rightarrow \bs})$ wherever $\det \partial_{\bmu} \bx^{\br}(\br)$ is large and vice-versa while $k \geq 0$ tunes the degree of penalisation. Since
%$$\left( \det \partial_{\br} \bs \right)^2 = \det G^{\br \rightarrow \bs} \leq \tfrac{1}{4} \left( \operatorname{tr} G^{\br \rightarrow \bs} \right)^2,$$
The contraction under $\sigma^k(\bx)$ has a similar effect as operating on $(\det \partial_{\br} \bs)^2$ directly while being inherently less prone to yielding degenerate discrete maps. In practice, the scheme converges reliably using Newton's method with line search for a wide range of choices $k > 0$ when the scheme is initialised with the tuple $(\bx^{\br}, \br)$ (i.e., the reference solution and reference controlmap). \\
\noindent We are again considering the screw geometry depicted with the bilinearly covered parametric domain before reparameterisation in Figure \ref{fig:male_screw_cell_k0}. Here, the reference solution corresponds to $\br(\bxi) = \bxi$.
\begin{figure}[h!]
\centering
\begin{subfigure}[b]{0.8 \textwidth}
    \includegraphics[width=0.45 \textwidth]{img/control/cell_size_hom/benchmark1_k0_param.png} \hfill
    \includegraphics[width=0.45 \textwidth]{img/control/cell_size_hom/benchmark1_k0.png}
    \caption{The reference geometry and controlmap.}
    \label{fig:male_screw_cell_k0}
\end{subfigure}
\\
\begin{subfigure}[b]{0.8 \textwidth}
    \includegraphics[width=0.45 \textwidth]{img/control/cell_size_hom/benchmark1_k2_param.png} \hfill
    \includegraphics[width=0.45 \textwidth]{img/control/cell_size_hom/benchmark1_k2.png}
    \caption{The screw geometry along with a plot of the corresponding controlmap $\bs: \hOm \rightarrow \hOm$ after reparameterisation with $k=2$.}
    \label{fig:male_screw_cell_k1}
\end{subfigure}
\caption{The screw geometry before and after reparameterisation under~\eqref{eq:cell_size_hom_diffusivity} with $k=2$.}
\label{fig:male_screw_cell_hom}
\end{figure}
\noindent Figure \ref{fig:male_screw_cell_hom} shows the geometry along with the associated controlmap $\bs(\bxi)$ after reparameterisation with $k=2$. Denoting the reparameterised maps by $\bx_h^k$, we define
$$\nu_{\text{Area}}^k := \frac{L_{\text{Area}}(\bx_h^k)}{L_{\text{Area}}(\bx_h^0)} \quad \text{and} \quad \nu_{\det J}^k := \frac{\sup \partial_{\bmu} \bx_h^k}{\inf \partial_{\bmu} \bx_h^k},$$
where the latter is approximated by sampling over the abscissae of a dense Gauss-Legendre quadrature scheme. 
\begin{table}
\renewcommand{\arraystretch}{1.5}
\centering
\begin{tabular}{c|c|c|c|c}
 k & 0 & 1 & 2 & 3 \\
 \hline
$\nu_{\text{Area}}^k$ & 1 & 0.749 & 0.680 & 0.649 \\
\hline
$\nu_{\det J}^k$ & 23.3 & 6.67 & 4.22 & 5.69
\end{tabular}
\caption{Table showing the ratios between evaluating~\eqref{eq:Area_multipatch} in $\bx^k_h$ and the reference evaluation in $\bx_h^0$ for various values of $k$ as well as the ratio of the maximum and minimum values of $\det \partial_{\bmu} \bx_h^k$ sampled over a dense quadrature scheme.}
\label{tab:poisson_area_ratio}
\end{table}

\noindent Table \ref{tab:poisson_area_ratio} contains the values of $\nu_{\text{Area}}^k$ and $\nu_{\det J}^k$ for various values of $k \in [0, 3]$. The table clearly demonstrates that the methodology has the desired effect, reaching saturation for larger values of $k$. Furthermore, all parameterisations with $k > 0$ significantly reduce the anisotropy of $\det \partial_{\bmu} \bx_h^k$. We mention that the diffusivity is merely essentially bounded since $\sigma^{k}(\bx^{\bs})$ is generally patchwise discontinuous. This may lead to singularities or unbounded growth (for an example of a scalar elliptic problem in which a diffusivity that is a scaling times the identity creates a singularity, see \cite{morin2002convergence, da2014mathematical}). However, in practice singularities are avoided and the problem requires no stabilisation. A possible explanation is that cell size homogenisation counteracts the tendency to generate singularities for discrete approximations. \\

\noindent As a second example, we are considering the geometry depicted in Figure \ref{fig:female_screw_reference_domain} (right) along with the parametric domain $\hOm$ given by a regular six-sided polygon. Unlike the geometry from Figure \ref{fig:male_screw_cell_k0}, this geometry has no corners. As such, we take $\hOmr$ to be the unit disc where the boundary correspondence $\mathbf{F}^{\bxi \rightarrow \br}: \partial \hOm \rightarrow \partial \hOmr$ is chosen such that the induced correspondence $\mathbf{F}^{\br \rightarrow \bx}: \partial \hOmr \rightarrow \partial \Om$ is diffeomorphic. The interior of $\hOmr$ is parameterised by applying the bilinearly-blended Coons' patch approach to each patch of $\hOm$ individually. The reference parameterisation $\bx^{\widehat{\br}}(\bxi): \hOm \rightarrow \Om$ and the associated reference controlmap $\widehat{\br}: \hOm \rightarrow \hOmr$ are depicted in Figure \ref{fig:female_screw_reference_domain}.
\begin{figure}[h!]
\centering
    \includegraphics[width=0.3 \textwidth, align=c]{img/control/interface_removal/female_screw/benchmark3_param_reference_reference.png}
    \includegraphics[width=0.3 \textwidth, align=c]{img/control/interface_removal/female_screw/benchmark3_param_reference.png}
    \includegraphics[width=0.3 \textwidth, align=c]{img/control/interface_removal/female_screw/benchmark3_geom_reference.png}
\caption{Depiction of $\hOm$, the parameterisation of $\hOmr$ under $\widehat{\br}: \hOm \rightarrow \hOmr$ and the reference parameterisation of $\Om$ under $\bx^{\widehat{\br}}(\bxi): \hOm \rightarrow \hOmr$.}
\label{fig:female_screw_reference_domain}
\end{figure}
\noindent In this example, we are combining the techniques from this section with those from Section \ref{subsect:interface_removal}. We employ the reference parameterisation $\widehat{\br}: \hOm \rightarrow \hOmr$ in combination with the diffusivity from~\eqref{eq:laplace_local_normalised_trace_penalty} to map $\hOmr$ onto itself. This results in the new reference controlmap $\br: \hOm \rightarrow \hOmr$ that removes the patch interfaces. The new parameterisation of $\hOmr$ and the associated new reference map $\bx^{\br}: \hOm \rightarrow \hOmr$ are depicted in Figure \ref{fig:female_screw_cell_k0}. Here, we do not stabilise using~\eqref{eq:patch_vertex_stabilisation} since the discrete approximation remains uniformly nondegenerate with acceptable behaviour in the vicinity of the patch vertices.
\begin{table}[h!]
\renewcommand{\arraystretch}{1.5}
\centering
\begin{tabular}{c|c|c|c|c|c}
 k & 0 & 1 & 2 & 3 & 4 \\
 \hline
$\nu_{\text{Area}}^k$ & 1.02 & 0.496 & 0.414 & 0.386 & 0.373  \\
\hline
$\nu_{\Gamma}^k$ & 0.117 & 0.142 & 0.158 & 0.171 & 0.180
\end{tabular}
\caption{Table showing the ratios between evaluating~\eqref{eq:Area_multipatch} in $\bx^k_h$ and the reference evaluation in $\bx_h^0$ for various values of $k$.}
\label{tab:female_poisson_area_interface_ratio}
\end{table}

\begin{figure}[h!]
\centering
\begin{subfigure}[b]{0.8 \textwidth}
    \includegraphics[width=0.45 \textwidth]{img/control/interface_removal/female_screw/benchmark3_param_k0.png} \hfill
    \includegraphics[width=0.45 \textwidth]{img/control/interface_removal/female_screw/benchmark3_geom_k0.png}
    \caption{$\bs(\hOm^{\br})$ and the female screw geometry after reparameterisation using~\eqref{eq:cell_size_hom_diffusivity} with $k=0$.}
    \label{fig:female_screw_cell_k0}
\end{subfigure}
\\
\begin{subfigure}[b]{0.8 \textwidth}
    \includegraphics[width=0.45 \textwidth]{img/control/interface_removal/female_screw/benchmark3_param_k4.png} \hfill
    \includegraphics[width=0.45 \textwidth]{img/control/interface_removal/female_screw/benchmark3_geom_k4.png}
    \caption{$\bs(\hOm^{\br})$ and the female screw geometry after reparameterisation using~\eqref{eq:cell_size_hom_diffusivity} with $k=4$.}
    \label{fig:female_screw_cell_k2}
\end{subfigure}
\caption{The female screw geometry after reparameterisation under~\eqref{eq:cell_size_hom_diffusivity} with $k=0$ and $k=4$.}
\label{fig:female_screw_cell_hom_local_trace_penalty}
\end{figure}
Table \ref{tab:female_poisson_area_interface_ratio} contains the values of
$$\nu^k_{\text{Area}} := \frac{L_{\text{Area}}(\bx^k_h)}{L_{\text{Area}}(\bx^{\widehat{\br}}_h)} \quad \text{and} \quad \nu^k_{\Gamma} := \frac{L_{\Gamma}(\bx_h^k)}{L_{\Gamma}(\bx^{\widehat{\br}}_h)}, \quad \text{with } L_{\Gamma}(\, \cdot \,) \text{ as in~\eqref{eq:interface_removal_norm}},$$
for various $k \in [0, 4]$. Figure \ref{fig:female_screw_cell_hom_local_trace_penalty} shows the parameterisation of the geometry for $k = 0$ and $k=4$. The table clearly demonstrates a monotonous reduction of $\nu^k_{\text{Area}}$ (eventually reaching saturation for larger values of $k$) at the expense of a slight increase in the value of $\nu^k_{\Gamma}$. \\

For more precise control over the expansion / contraction of cells, it can be helpful to decompose the diffusivity into the scaling $\sigma^k(\bx^{\bs})$ times the sum of two symmetric rank one tensors, i.e.,
\begin{align}
\label{eq:poisson_trace_penalty_general}
    D(\bx^{\bs}) = \frac{2}{a_i + 1} \sigma^k(\bx^{\bs}) \left( a_i \hat{\mathbf{v}}^{i, 1} \otimes \hat{\mathbf{v}}^{i, 1} + \hat{\mathbf{v}}^{i, 2} \otimes \hat{\mathbf{v}}^{i, 2} \right), \quad \text{ on } \br(\hat{\Omega}^i), \quad \text{where} \quad a_i > 0.
\end{align}
Here, $\hat{\mathbf{v}}^{i, 1}$ and $\hat{\mathbf{v}}^{i, 2}$ have length one and are not parallel. Note that
$$\operatorname{tr}\left(\frac{2}{a_i + 1}\left( a_i \hat{\mathbf{v}}^{i, 1} \otimes \hat{\mathbf{v}}^{i, 1} + \hat{\mathbf{v}}^{i, 2} \otimes \hat{\mathbf{v}}^{i, 2} \right) \right) = 2, \quad \text{as before}.$$
If the $\hat{\mathbf{v}}^{i, j}$ are patchwise discontinuous, we note that the diffusivity may require stabilisation. Taking $a_i$ large will force $\bs: \hOmr \rightarrow \hOmr$ to predominantly slide in the direction of $\mathbf{v}^{i, 1}$ on $\br(\hat{\Omega}^i)$.
\begin{figure}[h!]
\centering
\begin{subfigure}[b]{0.95 \textwidth}
    \includegraphics[width=0.3 \textwidth]{img/control/cell_size_hom/benchmark_3/benchmark3_param_reference.png} \hfill
    \includegraphics[width=0.3 \textwidth]{img/control/cell_size_hom/benchmark_3/benchmark3_param.png}
    \hfill
    \includegraphics[width=0.3 \textwidth]{img/control/cell_size_hom/benchmark_3/benchmark3_param_frozen.png}
    \caption{Visualisation of the reference controlmap (left) and the controlmaps $\bs: \hOmr \rightarrow \hOmr$ using $D(\br, \bx^{\bs}) = \sigma(\bx^{\bs})^k \mathcal{I}^{2 \times 2}$ and~\eqref{eq:poisson_trace_penalty_general}, both with $k = 3.5$. In the latter, $a_i$ is taken large close to $\partial \hOmr$ while $\hat{\mathbf{v}}^{i, 1}$ is the normalised component of $\partial_{\bmu} \br$ directed transversal to $\partial \hOmr$ for boundary patches.}
    \label{fig:throwing_star_cell_size_hom_param}
\end{subfigure}
\\
\begin{subfigure}[b]{0.95 \textwidth}
    \includegraphics[width=0.3 \textwidth]{img/control/cell_size_hom/benchmark_3/benchmark3_reference.png} \hfill
    \includegraphics[width=0.3 \textwidth]{img/control/cell_size_hom/benchmark_3/benchmark3_geometry.png} \hfill
    \includegraphics[width=0.3 \textwidth]{img/control/cell_size_hom/benchmark_3/benchmark3_geometry_frozen.png}
    \caption{The associated parameterisations. The parameterisations under Figure \ref{fig:throwing_star_cell_size_hom_param} (center) and Figure \ref{fig:throwing_star_cell_size_hom_param} (right) both show an outstanding homogenisation. The former exhibits a large degree of cell skewness close to the boundary, especially for the center left patch. Meanwhile, the latter avoids the boundary skewness but increases the isoline angles by the patch interfaces.}
    \label{fig:throwing_star_cell_size_hom_geom}
\end{subfigure}
\caption{Reparameterisation of a irregular geometry using $D(\br, \bx^{\bs}) = \sigma(\bx^{\bs})^k \mathcal{I}^{2 \times 2}$ (center) and~\eqref{eq:poisson_trace_penalty_general} (right). The latter avoids cell skewness close to the boundary. }
\label{fig:throwing_star_cell_size_hom}
\end{figure}
For large values of $k$, cell size homogenisation can lead to a considerable degree of cell skewness close to the boundary. As an example, Figure \ref{fig:throwing_star_cell_size_hom} (center) shows the homogenisation of a geometry with reference parameterisation depicted in Figure \ref{fig:throwing_star_cell_size_hom} (left) using~\eqref{eq:poisson_trace_penalty_general} under $D^{\bs}(\bx^{\bs}) = \sigma^k(\bx^{\bs}) \mathcal{I}^{2 \times 2}$ with $k=3.5$. This effect can be avoided by setting $\hat{\mathbf{v}}^{i, j} = \widehat{\partial}_{\bmu_j} \br$, where $\hat{\mathbf{v}}^{i, 1} = \widehat{\partial}_{\bmu^{\perp}} \br$ for boundary patches, while taking the $a_i$ large close to the boundary of $\hOmr$. The result for $k = 3.5$ is depicted in Figure \ref{fig:throwing_star_cell_size_hom} (right). With $\nu^k_{\text{Area}} = 0.515$ for the former and $\nu^k_{\text{Area}} = 0.518$ for the latter, the homogenisation is only marginally less effective under~\eqref{eq:poisson_trace_penalty_general}. However, the latter completely avoids cell skewness close to the boundary while sacrificing some regularity across the patch interfaces.


\subsection{Grid Adaptation}
\label{subsect:grid_adaptation}
In various applications it can be desirable to contract the map's isolines in regions where a large value of a function or its gradient is assumed. Given a function $f: \Om \rightarrow \mathbb{R}^{+}$, with $f \in C^{\infty}(\Om)$, the clustering of isolines can be achieved by designing diffusivities that contract the map's cell sizes in regions where $f: \Om \rightarrow \mathbb{R}^{+}$ is large (and vice-versa). The most basic choice is $D^{\bs}(\br, \bx) = \mathcal{I}^{2 \times 2}$ and $D^{\bx}(\bs, \bx) = \sigma(\bx) \mathcal{I}^{2 \times 2}$. With this choice $\bs(\bxi) = \br(\bxi)$ and~\eqref{eq:domain_optimization_coupled} is decoupled while the first equation can be regarded as the Euler-Lagrange equation of
\begin{align}
    \min \limits_{\br: \Om \rightarrow \hOmr} \int \limits_{\Om} \sigma(\bx) \operatorname{tr} \left( G^{\bx \rightarrow \br} \right) \mathrm{d} \bx \quad \text{s.t.} \quad \br = \left(\mathbf{F}^{\br \rightarrow \bx} \right)^{-1} \text{ on } \partial \Om,
\end{align}
where $G^{\bx \rightarrow \br}$ denotes the metric tensor of the map $\br(\bx): \Om \rightarrow \hOmr$. As such, minimisation will encourage the contraction of $\br(\bx)$ isolines in $\hOmr$ wherever $\sigma(\bx)$ is large and vice-versa. Exchanging the dependency $\br(\bx) \rightarrow \bx(\br)$, the isolines will now be contracted in regions where $\boldsymbol{\sigma}(\bx)$ is small. A possible choice for $\sigma(\bx)$ is \cite[Chapter~9]{liseikin1999grid}:
$$\sigma(\bx) = \frac{1}{\nu_1 f(\bx)^k + \nu_2}, \quad \text{or} \quad \sigma(\bx) = \frac{1}{\nu_1 \| \nabla f(\bx) \|^k + \nu_2} \quad \text{for gradient penalisation}.$$
Here, $\nu_2 > 0$ avoids division by zero in case $f \rightarrow 0$ and the parameters $\nu_1 > 0$ and $k > 0$ tune the degree of penalisation. A numerical scheme is best initialised with the nondegenerate reference solution (i.e., the solution for $\sigma(\bx) = 1$). \\
We are considering the screw geometry with reference parameterisation from Figure \ref{fig:male_screw_benchmark}. Here, we take $\br(\bxi) = \bxi$ and $\hOmr = \hOm$. We would like to contract cells based on the function value of a ring-shaped function $f \in C^{\infty}(\Om)$ using $\nu_1 = 1$, $\nu_2 = 0.01$ and $k = 1$. Figure \ref{fig:male_screw_adaptivity_Id} depicts the result of reparameterising under $D^{\bx}(\bx)$ along with an arrow plot showing the movement of a select number of points with respect to the reference map.
\begin{figure}[h!]
\centering
\includegraphics[height=7.5cm]{img/control/adaptivity/adaptivity0_Id.png} \hspace*{0.1cm}
\includegraphics[height=6.8cm]{img/control/adaptivity/adaptivity0_Id_arrows.png}
\caption{Figure showing the cell size contraction in the vicinity of large function values of a ring-shaped function $f \in C^{\infty}(\Om)$. The arrows in the right figure show the movement of select points with respect to the reference parameterisation from Figure \ref{fig:male_screw_benchmark_geom}.}
    \label{fig:male_screw_adaptivity_Id}
\end{figure}
\noindent The figure shows a strong contraction of cells in the vicinity of large function values, clearly demonstrating that the methodology has the desired effect. The cell contraction can be increased by increasing the value of $\nu_1$ or $k$. However, strong penalisation can have unpredictable effects on the cells, in particular close to the patch vertices. \\
In practice, this can be avoided by performing patch interface removal using the techniques of Section \ref{subsect:interface_removal}. We are considering the same example as before while now performing interface removal with stabilisation in $\hOmr$. Figure \ref{fig:male_screw_adaptivity_Id_smooth} shows the images of locally drawn isolines in $\hOmr$ along with the result of performing cell contraction using the same parameters.
\begin{figure}[H]
\centering
\includegraphics[height=6.8cm]{img/control/adaptivity/adaptivity0_Id_smooth_param.png} \hspace*{0.1cm}
\includegraphics[height=6.8cm]{img/control/adaptivity/adaptivity0_Id_smooth.png}
\caption{Figure showing the parameterisation of $\hOmr = \hOm$ and the result of performing cell size contraction under the coordinate transformation.}
    \label{fig:male_screw_adaptivity_Id_smooth}
\end{figure}
Compared to Figure \ref{fig:male_screw_adaptivity_Id}, isolines crossing the patch interfaces exhibit less erratic behaviour and align well with the ring-shaped function. \\
To demonstrate that the proposed technique (in combination with interface removal) is effective when applied to geometries with fewer symmetries than in Figure \ref{fig:male_screw_adaptivity_Id}, we refer to Figure \ref{fig:throwing_star_adaptivity_Id_smooth}.
\begin{figure}[H]
\centering
\includegraphics[height=6.8cm]{img/control/adaptivity/adaptivity_1_Id_smooth_param.png} \hspace*{0.1cm}
\includegraphics[height=6.8cm]{img/control/adaptivity/adaptivity_1_Id_smooth.png}
\caption{A further example of grid adaptation in the vicinity of large function values with interface removal.}
    \label{fig:throwing_star_adaptivity_Id_smooth}
\end{figure}

% \subsection{Boundary orthogonality and Boundary Layers}
% Many applications favour a parameterisation with isolines that intersect the boundary $\partial \Om$ at a right angle. In the singlepatch setting, \cite{hinz2020goal} adopts the method from \cite[Chapter 4]{thompson1998handbook} and alters it for compatibility with IGA. More precisely, the method seeks the four functions $f_s(\, \cdot \,), f_n(\, \cdot \,), g_e(\, \cdot \,)$ and $g_w(\, \cdot \,)$ such that the controlmap $\bs: \Om^{\square} \rightarrow \Om^{\square}$ defined as
% $$\bs_1(\mu_1, \mu_2) = f_s(\mu_1) H_0(\mu_2) + f_n(\mu_1) H_1(\mu_2) \quad \text{and} \quad \bs_2(\mu_1, \mu_2) = g_e(\mu_2) H_0(\mu_1) + g_w(\mu_2) H_1(\mu_1)$$
% with $H_0(x) = (1 + 2x) (1 - x)^2$ and $H_1(x) = (3 - 2 x)x^2$, is orthogonal at a user-specified subset of the four sides of $\partial \Om^{\square}$. Denoting by $\gamma_e, \gamma_w, \gamma_s$ and $\gamma_n$ the eastern, western, southern and northern sides of $\partial \Om^{\square}$, respectively, to find $f_s$ and $f_n$, for instance, the method solves the discrete counterpart of the mixed Dirichlet-Neumann problem
% $$\Delta f = 0 \text{ in } \Om, \quad \text{s.t. } f = 0 \text{ on } \gamma_e, \, f = 1 \text{ on } \gamma_w \text{ and } \frac{\partial f}{\partial \mathbf{n}} = 0 \text{ on } \gamma_s \cup \gamma_n$$
% using an initially nondegenerate reference map $\bx_h^{*}: \Om^{\square} \rightarrow \Om$. The functions are then either defined as $i \in \{s, n\}$ $f_i(\mu_1) = \mu_1$ if orthogonality at $\gamma_i$ is not desired or $f_s(\, \cdot \,) = f(\, \cdot \,, 0)$, respecively $f_n(\, \cdot \,) = f(\, \cdot \,, 1)$, else. The corresponding functions $g_{e}$ and $g_w$ are found by exchanging the roles $f \rightarrow g$, $\{\gamma_e, \gamma_w\} \rightarrow \{\gamma_s, \gamma_n\}$ (and vice-versa) and $\{ \mu_1, \mu_2 \} \rightarrow \{\mu_2, \mu_1\}$. If the underlying spline basis is bicubic, the controlmap can be exactly expressed as a spline surface over $\mathcal{V}_h^2$, else, it can be approximated in the least squares sense. Here, the Hermite interpolation functions $H_0(\, \cdot \,)$ and $H_1(\, \cdot \,)$ ensure that the directional derivative of the recomputed map's tangent component vanishes in the transverse direction, i.e., for instance, \smash{$\partial_{\mu_2} \bx_1^{\bs} = 0$} on $\gamma_s$. While a generalisation to the multipatch setting may be possible, the aforementioned transverse requirement would lead to complicated polynomial constructions in $\hOm$, which are beyond the scope of this paper. \\
% As the reference map $\bx_h^{*}(\bxi)$ naturally divides into $N_p$ singlepatch maps via the composition with the \smash{$\bm^i: \Om^{\square} \rightarrow \hOm_i$}, a convenient way of achieving orthogonality on specified boundary (and interior) facets is applying the singlepatch methodology patchwise. Hereby, the singlepatch boundaries follow naturally from the restriction of $\bx_h^{*}$ to the facets of $\hOm$. As the cardinality of each singlepatch problem is given by the much lower cardinality of the local spline basis in $\Om^{\square}$, the complexity of orthogonalising patchwise is low. Heuristically, the best results are obtained by constructing a reference map \smash{$\bx_h^{*}$} that uses a controlmap \smash{$\bs: \hOmr \rightarrow \hOm^{\bs}$} based on the techniques from Section \ref{subsect:interface_removal}. It should be noted that facets  \\
% We are considering the screw geometry along with the reference parameterisation and controlmap from Figure \ref{fig:male_screw_interface_remove_k0} and apply orthogonalisation to the boundary facets only. The resulting parameterisation is depicted in Figure \ref{fig:male_screw_boundary_orth_1_map}. We can reconstruct the reference controlmap $\br: \hOm \rightarrow \hOm$ that would generate this map by solving the discretised counterpart of~\eqref{eq:find_controlmap_given_x}. The result for the boundary correspondence $\mathbf{F}^{\bxi \rightarrow \br}(\bxi) = \bxi$ is depicted in Figure \ref{fig:male_screw_boundary_orth_1_controlmap}.
% \begin{figure}[h!]
% \centering
% \begin{subfigure}[b]{0.4 \textwidth}
%     \includegraphics[width=\textwidth]{img/control/boundary_orth/benchmark1_controlmap.png}
%     \caption{Depiction of the controlmap that would produce the parameterisation from \ref{fig:male_screw_boundary_orth_1}.}
%     \label{fig:male_screw_boundary_orth_1_controlmap}
% \end{subfigure}
% \hspace*{1cm}
% \begin{subfigure}[b]{0.4 \textwidth}
%     \includegraphics[width=\textwidth]{img/control/boundary_orth/benchmark1.png}
%     \caption{The screw parameterisation orthogonalised by the boundaries.}
%     \label{fig:male_screw_boundary_orth_1_map}
% \end{subfigure}
% \caption{The screw geometry from Figure \ref{fig:male_screw_interface_remove_k0} orthogonalised by the boundaries (b) along with the corresponding controlmap obtained by solving~\eqref{eq:find_controlmap_given_x}.}
% \label{fig:male_screw_boundary_orth_1}
% \end{figure}
% The figure shows outstanding boundary orthogonalisation. However, since applying orthgononalisation patchwise does not allow for control across patch interfaces, the suppression of transverse jumps across interfaces is lost.

\subsection{Boundary Orthogonality}
\label{subsect:boundary_orthogonality}
Many applications favour a parameterisation in which locally drawn $\bmu$-isolines intersect the boundary $\partial \Omega$ at a right angle. Unfortunately, it is not possible to simultaneously impose Dirichlet and Neumann data on the inverted elliptic equations. As such, boundary orthogonality has to be enforced through an appropriate coordinate transformation in the parametric domain $\hOmr$, wherein we assume $\hOmr = \hOm$ for convenience. Furthermore, we assume that each $\overline{\Om_i}$ coincides on $\partial \Om$ with exactly one of the curves $\overline{C}_K$. Here, we give a multipatch generalisation of the singlepatch method proposed in \cite{hinz2020goal}. Given the reference solution $\bx_h: \hOm \rightarrow \Om$ over the original bilinearly covered parametric domain $\hOm$, we introduce the maps 
$$\bx_h^i(\bmu) := \bx_h \circ \bm^i, \quad \text{for boundary patches } \hOm_i \in \mathcal{Q}^B$$
and we denote $\bx_h^i(\Om^{\square}) := \Omega_i \subset \Omega$. Without loss of generality, we may assume that each $\hOm_i$ is oriented such that $\mu_1$ and $\mu_2$ correspond to the directions tangential and transversal to $\partial \Omega$, respectively. Denoting the eastern, western, southern and northern segments of $\partial \Om^\square$ by $\gamma_e, \gamma_w, \gamma_s$ and $\gamma_n$, respectively, we may furthermore assume the orientation is such that $\gamma_n$ is mapped onto $C_k \subset \partial \Omega$ under $\bx_h^i$. We denote the associated sides of $\Om_i$ under the map $\bx_h^i$ by $\Gamma_e^i, \Gamma_w^i, \Gamma_s^i$ and $\Gamma_n^i = C_k \subset \partial \Omega$. We are seeking a function $f_i: \Omega_i \rightarrow \mathbb{R}$ that satisfies homogeneous Neumann boundary conditions on $\Gamma_n^i$. For this, we solve
$$\Delta f_i = 0 \text{ in } \Om_i, \quad \text{s.t.} \quad f_i(\bx(\bmu)) = \mu_1 \text{ on } \overline{\Gamma_e^i} \cup \overline{\Gamma_w^i} \cup \overline{\Gamma_s^i} \quad \text{and} \quad \frac{\partial f_i}{\partial \mathbf{n}} = 0 \text{ on } \Gamma_n^i,$$
where $\mathbf{n}$ denotes the unit outward normal vector on $\partial \Omega_i$. A pullback leads to
$$\Delta_{\bx_h^i} f_i = 0 \text{ in } \Om^\square, \quad \text{s.t.} \quad f_i(\bmu) = \mu_1 \text{ on } \overline{\gamma_e} \cup \overline{\gamma_w} \cup \overline{\gamma_s} \quad \text{and} \quad \frac{\partial f_i}{\partial \mathbf{n}} = 0 \text{ on } \gamma_n,$$
whose discretisation imposes the Neumann data through partial integration in the usual way. The restriction $q_i(\mu_1) := f_i \vert_{\gamma_n}$ will be a monotone function over $\mu_1 \in [0, 1]$ thanks to the imposed Dirichlet data and the maximum principle. Given a diffeomorphism $\bnu^i: \Om^{\square} \rightarrow \Om^{\square}$ that satisfies $\bnu^i \vert_{\gamma_n} = q_i$ and $\partial_{\mu_2} \bnu^i_1 = 0$ on $\gamma_n$, a map $\tilde{\bx}^i: \Om^{\square} \rightarrow \Omega_i$ that maps inversely harmonically into $\Omega^{\square}$ with the coordinate system induced by $\bnu^i$, will map local $\mu_1$ isolines onto isolines in $\Omega_i$ that intersect $\overline{C_k} = \partial \Omega \cap \overline{\Omega}_i$ at a right angle, thanks to the Neumann data we imposed on $\Gamma_n^i$. Two possible choices are given by
\begin{align}
\label{eq:boundary_orth_mu1_functions}
    \bnu^i_1(\bmu) = q_i(\mu_1) \quad \text{and} \quad \bnu^i_1(\bmu) = t_i(\bmu) \quad \text{with} \quad t_i(\bmu) := (1 + 2 \mu_2) \, (1 - \mu_2)^2 \, \mu_1 + (3 - 2 \mu_2) \, \mu_2^2 \, q_i(\mu_1),
\end{align}
while $\bnu^i_2(\bmu) = \mu_2$. Here, the former maps straight $\mu_1$ isolines onto straight $q_i(\mu_1)$ isolines in $\Om^{\square}$ while the latter maps the same isolines onto curves that start at $\bmu = (\mu_1, 0)$ and end in $\bmu = (q_i(\mu_1), 1)$ while intersecting $\gamma_n$ at a right angle. Note that the latter furthermore satisfies $\bnu^i(\bmu) = \bmu$ on $\gamma_s$. \\
With this choice of $\bnu^i$, a map $\tilde{\bx}: \hOm \rightarrow \Om$ that maps inversely harmonically into $\hOm$ with the coordinate system induced by the controlmap $\bs: \hOm \rightarrow \hOm$ that satisfies 
$$\bs(\bmu) = \bm^i \circ \bnu^i, \quad \text{or equivalently} \quad \bs(\bxi) = \bm^i \circ \bnu^i \circ (\bm^i)^{-1} \quad \text{on} \quad \hOm_i \in \mathcal{Q}^B,$$
will now map the images of local $\mu_1$-isolines under $\bm^i$ onto isolines in $\Om_i$ that intersect $\partial \Omega$ at a right angle. The controlmap $\bs: \hOm \rightarrow \hOm$ that leads to boundary orthogonality is hence known for boundary patches $\hOm_i \in \mathcal{Q}^B$. For the choice $\bnu^i_1(\bmu) = t_i(\bmu)$, the controlmap $\bs: \hOm \rightarrow \hOm$ can be taken as the identity on patches $\hOm_k \notin \mathcal{Q}^B$. \\
For the choice $\bnu^i_1 = q_i(\mu_1)$, on the other hand, the partially-known controlmap induces a reparameterisation of the interior facets $\gamma_{ij} \in \Gamma^I$ with $\hOm_i \in \mathcal{Q}^B$ or $\hOm_j \in \mathcal{Q}^B$. As such, the original bilinear parameterisations of patches $\hOm_k \notin \mathcal{Q}^B$ will no longer be conforming to the images of boundary patches under $\bs(\bxi)$. In this case, we may require the controlmap to satisfy $\bs(\bxi) \vert_{\gamma_{ij}} = \bxi$ for facets $\gamma_{ij} \in \Gamma^I$ that are not associated with one of the boundary patches. With that, the map $\bs: \hOm \rightarrow \hOm$ is now known on the boundary patches and on all interior facets. The interior of the remaining patches $\hOm_k \notin \mathcal{Q}^B$ can now be parameterised from the curves $\bs \vert_{\gamma_{ij}}, \, \gamma_{ij} \in \Gamma^I$ one-by-one using, for instance, the bilinearly-blended Coons' patch approach. The result is a controlmap $\bs: \hOm \rightarrow \hOm$ that leads to boundary orthogonality and is furthermore conforming across all interior facets. \\
The controlmap can be projected onto $\mathcal{V}_h^2$, where we note that for $\bnu^i_1 = t_i(\bmu)$, $\mathcal{V}_h$ has to be patchwise bicubic in order for the projection to be exact. \\
We are again considering the screw geometry whose reference controlmap and parameterisation are depicted in Figure \ref{fig:male_screw_cell_k0}. As a measure for the degree of boundary orthogonalisation, we utilise
\begin{align}
    L_{\perp}^2(\bx) := \sum \limits_{\hOm_i \in \mathcal{Q}^B} \, \int \limits_{\partial \hOm \cap \overline{\hOm}_i} \left(\widehat{\partial}_{\bmu^{\perp}} \bx \cdot \widehat{\partial}_{\bmu^\parallel} \bx \right)^2 \mathrm{d} \Gamma,
\end{align}
wherein $\widehat{\partial}_{\mu^{\parallel}}( \, \cdot \, )$ and $\widehat{\partial}_{\mu^{\perp}}( \, \cdot \, )$ denote the normalised tangential and transverse derivatives with respect to $\bmu$ on $\hOm_i \in \mathcal{Q}^B$, respectively. \\
Figure \ref{fig:male_screw_boundary_orth_geom} shows the reparameterisations of $\hOm$ under $\bs: \hOm \rightarrow \hOm$ for the choices $\bnu^i_1(\bmu) = q_i(\mu_1)$ and $\bnu^i_1(\bmu) = t_i(\bmu)$, respectively, while Figure \ref{fig:male_screw_boundary_orth_geom} shows the associated parameterisations of $\Om$ after recomputation under $\bs: \hOm \rightarrow \hOm$.
\begin{figure}[h!]
\centering
\begin{subfigure}[b]{0.8 \textwidth}
    \includegraphics[width=0.45 \textwidth]{img/control/boundary_orth/straight/male_screw_straight_param.png} \hfill
    \includegraphics[width=0.45 \textwidth]{img/control/boundary_orth/straight/male_screw_not_straight_param.png}
    \caption{Reparameterisation of $\hOm$ under $\bs: \hOm \rightarrow \hOm$ with the choices $\bmu_1^i(\bmu) = q_i(\mu_1)$ (left) and $\bmu_1^i(\bmu) = t_i(\bmu)$ (right).}
    \label{fig:male_screw_boundary_orth_param}
\end{subfigure}
\\
\begin{subfigure}[b]{0.8 \textwidth}
    \includegraphics[width=0.45 \textwidth]{img/control/boundary_orth/straight/male_screw_straight_geom.png} \hfill
    \includegraphics[width=0.45 \textwidth]{img/control/boundary_orth/straight/male_screw_not_straight_geom.png}
    \caption{The parameterisations of $\Om$ under the controlmaps from \textbf{(a)}.}
    \label{fig:male_screw_boundary_orth_geom}
\end{subfigure}
\caption{}
\label{fig:male_screw_orth}
\end{figure}
With
$$\frac{L_{\perp}(\bx^{\bs})}{L_{\perp}(\bx^{\bxi})} = 0.172 \quad \text{for} \quad \bmu_1^i(\bmu) = q_i(\mu_1) \quad \text{and} \quad \frac{L_{\perp}(\bx^{\bs})}{L_{\perp}(\bx^{\bxi})} = 0.169 \quad \text{for} \quad \bmu_1^i(\bmu) = t_i(\bmu),$$
both choices are similarly effective, wherein the small discrepancy is explained by differing truncation errors. Figure \ref{fig:male_screw_boundary_orth_geom}, left, reveals that the choice $\bmu_1^i(\bmu) = q_i(\mu_1)$ leads to a strong clustering of cells close to the patch interfaces, which may not be desirable. This is not the case for \ref{fig:male_screw_boundary_orth_geom}, right. Meanwhile, the former maps straight isolines in $\Om^{\square}$ onto straight isolines on the $\hOm_i \in \mathcal{Q}^B$, a property that can be exploited when combining boundary orthogonalisation with the creation of a boundary layer (see Section \ref{subsect:boundary_layers}).

\subsection{Boundary layers}
\label{subsect:boundary_layers}
Many applications in computational fluid dynamics deal with PDE-problems whose solutions are known to create a steep gradient in the vicinity of the boundary $\partial \Om$. To capture important features of the solution, such applications favour parameterisations with a dense clustering of cells in the vicinity of $\partial \Omega$. This can be achieved by introducing a controlmap $\bs: \hOm \rightarrow \hOm$ that clusters locally-drawn $\bmu$-isolines close to $\partial \hOm$, while potentially sacrificing some cell density in the interior. We assume that $\hOmr = \hOm$ is a regular $2n$-sided polygon with radius one, centered at $\bxi = (0, 0)^T$. As before, we assume that $\mu_1 = \text{const}$ refers to the local $\bmu$-direction transverse to $\partial \hOm$ for boundary patches. A convenient way to create a boundary layer is utilising a diffusivity of the form
\begin{align}
\label{eq:boundary_layer_diffusivity}
    D^{\bs}(\bxi) = (1 - \exp{(-\mu \|\bxi \|^2)}) \, \| \bxi \|^k \, \left( \hat{\bxi} \otimes \hat{\bxi} \right) + \nu \mathcal{I}^{2 \times 2},
\end{align}
for some $\mu \gg 1$, $\nu \ll 1$ and $k > 0$. Here, $\hat{\bxi} := \bxi / \| \bxi \|$ while the prefactor $(1 - \exp{(-\mu \|\bxi \|^2)})$ in~\eqref{eq:boundary_layer_diffusivity} avoids the singularity in the origin. Taking $\nu$ small urges the controlmap $\bs: \hOm \rightarrow \hOm$ to map points $\bxi \in \hOm$ in radially outward direction with a tight clustering close to $\partial \hOm$. If the locally-drawn $\mu_1$ isolines of boundary patches $\hOm_i \in \mathcal{Q}^B$ align with straight rays drawn from the origin in radially outward direction as in Figure \ref{fig:male_screw_cell_k0}, the diffusivity from~\eqref{eq:boundary_layer_diffusivity} will furthermore largely preserve the intersection angle of the $\mu_1$ isolines with the boundary $\partial \Omega$ (w.r.t. to the choice $D^{\bs} = \mathcal{I}^{2 \times 2}$). Since the controlmap creation is an a priori step, the methodology is compatible with all operators from Section \ref{sect:numerical_schemes}. \\
We are considering the screw geometry with the reference parameterisation from Figure \ref{fig:male_screw_cell_k0}. Figure \ref{fig:male_screw_boundary_layer_vanilla} shows the reparameterisation using~\eqref{eq:boundary_layer_diffusivity} with $\mu = 30$, $k = 2$ and $\nu = 0.005$.
\begin{figure}[H]
\centering
\includegraphics[height=6.8cm]{img/control/boundary_layers/male_screw_k2_nu005_param.png} \hspace*{0.1cm}
\includegraphics[height=6.8cm]{img/control/boundary_layers/male_screw_k2_nu005_geom.png}
\caption{Example showing the creation of a boundary layer using~\eqref{eq:boundary_layer_diffusivity} with $\mu = 30$, $k=2$ and $\nu = 0.005$.}
\label{fig:male_screw_boundary_layer_vanilla}
\end{figure}
The figure shows a strong clustering of transverse isolines close to the boundary. The clustering intensity can be increased by increasing the value of $k$. \\
As a second example, we are considering the female screw geometry with reference controlmap and parameterisation shown in Figure \ref{fig:female_screw_reference_domain}. While $\hOmr \neq \hOm$ is now given by the unit disc, the boundary patches are oriented such that the $\mu_1$ transverse isolines align with straight rays that intersect the origin, as required. As such, we replace $\bxi \rightarrow \br$ in~\eqref{eq:boundary_layer_diffusivity} and expect the diffusivity to largely preserve the intersection angle of transverse isolines with $\partial \hOmr$ and $\partial \Om$. Figure \ref{fig:female_screw_boundary_layer_vanilla} shows the result of boundary layer creation under~\eqref{eq:boundary_layer_diffusivity} using the same parameters as in Figure \ref{fig:male_screw_boundary_layer_vanilla}.
\begin{figure}[H]
\centering
\includegraphics[height=6.8cm]{img/control/boundary_layers/female_screw_k2_nu005_param.png} \hspace*{0.1cm}
\includegraphics[height=6.8cm]{img/control/boundary_layers/female_screw_k2_nu005_geom.png}
\caption{Example showing the creation of a boundary layer using~\eqref{eq:boundary_layer_diffusivity} with $\mu = 30$, $k=2$ and $\nu = 0.005$.}
\label{fig:female_screw_boundary_layer_vanilla}
\end{figure}
In both examples, the layer density is intensified / reduced close to the inward-facing and protruded parts of $\partial \Omega$, respectively. This effect may be counteracted by introducing a position-dependent clustering parameter, i.e., $k \rightarrow k(\br)$. However, this is beyond the scope of this paper. \\
As a final example, we are combining boundary layer creation with boundary orthogonality. For this purpose, we assume that we are in the possession of a controlmap $\bs: \hOm \rightarrow \hOm$ that orthogonalises transverse $\mu_1$ isolines for boundary patches $\hOm_i \in \mathcal{Q}^B$. Assuming again that the orientation is chosen such that the transverse direction is given by $\mu_1 = \text{const}$ for the $\hOm_i \in \mathcal{Q}^B$, we restrict ourselves to the choice $\bnu_1^i(\bmu) = q_i(\mu_1)$ (cf.~\eqref{eq:boundary_orth_mu1_functions}) such that $\bs: \hOm \rightarrow \hOm$ maps straight $\mu_1$ isolines onto straight $\mu_1$ isolines for boundary patches, as in Figure \ref{fig:male_screw_boundary_orth_param} (left). For the purpose of boundary layer creation, we may compose the $\bnu^i(\bmu) = (q_i(\mu_1), \mu_2)^T$ with a function of the form $\blambda^i(\bmu) = (\mu_1, f_i(\mu_1, \mu_2))^T$, where $f_i(\mu_1, 0) = 0$, $f_i(\mu_1, 1) = 1$ and $\partial_{\mu_2} f_(\mu_1, \mu_2) > 0$. We note that the map $\blambda^i \circ \bnu^i: \Om^{\square} \rightarrow \Om^{\square}$ still satisfies $\partial_{\mu_2} (\blambda^i \circ \bnu^i )_1 = 0$ on $\gamma_n$ such that boundary orthogonality is preserved. The purpose of $f_i$ is to create a boundary layer near $\mu_2 = 1$, i.e., $\partial_{\mu_2} f_i(\mu_1, \mu_2)$ in $\mu_2 = 1$ should be small. A function that satisfies aforementioned requirements is given by
\begin{align}
    f_i(\mu_1, \mu_2) = \frac{1 - \exp{(-d_i(\mu_1) \mu_2)}}{1 - \exp{(-d_i(\mu_1))}}, \quad \text{ for some } \quad d_i(\mu_1) > 0,
\end{align}
where larger values of $d_i(\mu_1)$ create a (locally) stronger boundary layer. Note that we have
\begin{align}
    \left. \partial_{\mu_2} f_i(\mu_1, \mu_2) \right \vert_{\gamma_n} := f^{\prime}_{i, n}(\mu_1) = \frac{d_i(\mu_1) \exp{(-d_i(\mu_1))}}{1 - \exp{(-d_i(\mu_1))}}.
\end{align}
Thanks to boundary orthogonalisation, the local tangent bundle of $\bx^{\bs}$ is diagonal in the basis that is spanned by the unit tangent and normal vectors on $\partial \Omega$, i.e,
\begin{align}
\label{eq:boundary_layer_local_tangent_bundle_diagonal}
    \partial_{\bmu} \bx^{\bs} = a_i \mathbf{t} \otimes \mathbf{t} + b_i \mathbf{n} \otimes \mathbf{n}, \quad \text{on} \quad L_{k^i} := \overline{\hOm_i} \cap \partial \Omega \quad \text{for } \hOm_i \in \mathcal{Q}^B,
\end{align}
where $a_i$ follows from the boundary correspondence $\mathbf{F}: \partial \hOm \rightarrow \partial \Om$ while $b_i$ is a property of the parameterisation of the interior. We would like to create a new controlmap $\tilde{\bs}: \hOm \rightarrow \hOm$ whose associated map $\bx^{\tilde{\bs}}: \hOm \rightarrow \Om$ satisfies
\begin{align}
    \partial_{\bmu} \bx^{\tilde{\bs}} = a_i \mathbf{t} \otimes \mathbf{t} + k \mathbf{n} \otimes \mathbf{n} \quad \text{on} \quad L_{k^i} := \overline{\hOm_i} \cap \partial \Omega \quad \text{for } \hOm_i \in \mathcal{Q}^B,
\end{align}
where $k > 0$ is a user-specified parameter. Requiring $\tilde{\bs}: \hOm \rightarrow \hOm$ to be of the form
\begin{align}
\label{eq:orth_boundary_layer_controlmap_boundary_patches}
    \tilde{\bs}(\bxi) = \bm^i \circ \blambda^i \circ \bnu^i  \circ (\bm^i)^{-1} \quad \text{on } \hOm_i \in \mathcal{Q}^B,
\end{align}
it is clear that the recomputed map will satisfy
\begin{align}
    \left. \partial_{\bmu} \bx^{\tilde{\bs}}(\bmu) \right \vert_{\gamma_n} = a_i(\mu_1) \mathbf{t} \otimes \mathbf{t} + b_i(\mu_1) f_{i, n}^{\prime}(\mu_1) \mathbf{n} \otimes \mathbf{n} \quad \text{on} \quad L_{k^i} \subset \partial \hOm \quad \text{for } \hOm_i \in \mathcal{Q}^B.
\end{align}
Given that each $f_{i, n}^{\prime} = f_{i, n}^{\prime}(d_i)$, we may find the $d_i(\mu_1)$ by minimising the nonlinear cost function
\begin{align}
\label{eq:constant_transverse_deriv_opt}
    \sum \limits_{\{i \, \vert \, \hOm_i \in \mathcal{Q}^B \}} \, \, \int \limits_{L_{k^i}} (b_i f^{\prime}_{i, n} -k )^2 \mathrm{d} \Gamma \rightarrow \min \limits_{d},
\end{align}
where $b_i$ and $f^{\prime}_{i, n}$ are now taken as functions over $\bxi \in L_{k^i} \subset \partial \hOm$ while $d: \partial \hOm \rightarrow \mathbb{R}$ satisfies
\begin{align}
    d(\bxi) = d_i \circ (\mathbf{m}^i)^{-1} \quad \text{on } L_{k^i} \subset \partial \hOm.
\end{align}
A discretisation then constructs $d(\bxi)$ from the linear span of the $\phi_h \in \mathcal{V}_h$ that are nonvanishing on $\partial \hOm$ and finds the minimum over this subspace of $C^0(\partial \hOm)$ using Newton's method. Upon completion, the function $d(\bxi)$ is known on $\partial \hOm$ and the restriction to $L_{k^i} \subset \partial \hOm$ can be expressed as a function over $\gamma_n \subset \partial \Om^{\square}$ via the $(\mathbf{m}^i)^{-1}$. The canonical extension from $\gamma_n$ into $\Om^{\square}$ then defines $\blambda^i(\bmu) = (\mu_1, f_i(\mu_1, \mu_2))^T$ and we define $\tilde{\bs}: \hOm \rightarrow \hOm$ by~\eqref{eq:orth_boundary_layer_controlmap_boundary_patches} for boundary patches while requiring $\tilde{\bs}(\bxi) = \bs(\bxi)$ for interior patches. Since $d(\bxi) \in C^0(\partial \hOm)$, the controlmap defined in this way will be conforming across all interior interfaces. Finally, to relieve the computational burden, the controlmap $\tilde{\bs}: \hOm \rightarrow \hOm$ is expressed in $\mathcal{V}_h^2$ via an $L^2(\hOm)$ projection. \\

\noindent We are considering the screw geometry with orthogonalised reference parameterisation from Figure \ref{fig:male_screw_boundary_orth_geom} (left) and associated controlmap $\bs: \hOm \rightarrow \hOm$ from Figure \ref{fig:male_screw_boundary_orth_param} (left). Using this reference parameterisation, we are creating a boundary layer in which value of $k > 0$ in~\eqref{eq:constant_transverse_deriv_opt} is given by $\overline{b} / 72$, where $\overline{b}$ is the average value of all $b_i$ over all $L_{k^i}$ in~\eqref{eq:boundary_layer_local_tangent_bundle_diagonal}. Figure \ref{fig:male_screw_boundary_layer_algebraic} shows the resulting parameterisation along with the controlmap $\tilde{\bs}: \hOm \rightarrow \hOm$, while Figure \ref{fig:male_screw_boundary_layer_algebraic_zoom} shows a zoom-in on two different segments on the boundary.
\begin{figure}[H]
\centering
\includegraphics[height=6.8cm]{img/control/boundary_layers/algebraic/male_screw_orth_exp_scaled_k05_param.png} \hspace*{0.1cm}
\includegraphics[height=6.8cm]{img/control/boundary_layers/algebraic/male_screw_orth_exp_scaled_k05_geom_labeled.png}
\caption{Controlmap and the associated parameterisation of the male screw geometry orthogonalised by the boundaries along with a boundary layer that has been created using a sequence of algebraic operations on the boundary patches. Figure \ref{fig:male_screw_boundary_layer_algebraic_zoom} shows a zoom-in on the segments that have been highlighted in the right figure.}
\label{fig:male_screw_boundary_layer_algebraic}
\end{figure}
\begin{figure}[H]
\centering
\includegraphics[height=4cm]{img/control/boundary_layers/algebraic/male_screw_orth_exp_scaled_k05_geom_zoom.png} \hspace*{0.1cm}
\includegraphics[height=3cm]{img/control/boundary_layers/algebraic/male_screw_orth_exp_scaled_k05_geom_zoom3.png}
\caption{A zoom-in on two different segments of the boundary showing the boundary orthogonalisation as well as the boundary layer that is largely maintained along the entire boundary.}
\label{fig:male_screw_boundary_layer_algebraic_zoom}
\end{figure}
As can be seen, the methodology preserves the boundary orthogonalisation while now providing precise control over the density of the boundary layer, which is largely maintained along the entire boundary. As before, the boundary layer density is tuned by the value of $k > 0$. Since the method performs a sequence of algebraic operations on the boundary patches, unlike in the previous methodology, the interior patches remain unchanged. As such, the best results are obtained when the boundary patches cover the majority of $\partial \hOm$ with only a handful of small patches in the interior.
% \subsection{Boundary layers}
% \label{subsect:boundary_layers}
% Some applications require a parameterisation with a dense clustering of $\bmu$-isolines in the vicinity of the domain's boundary. This can be accomplished by introducing a diffusivity of the form
% \begin{align}
%     D^{\bs}(\br, \bx^{\bs}) = a_i(\br) \widehat{\partial}_{\mu^{\perp}} \br \otimes \widehat{\partial}_{\mu^{\perp}} \br + \mathcal{I}^{2 \times 2} \quad \text{on } \br(\hOm_i), \text{ for boundary patches } \hOm_i.
% \end{align}
% As before, $\widehat{\partial}_{\mu^{\perp}} \br$ denotes the normalised local directional derivative transversal to $\partial \hOm^{\br}$. For interior patches, we simply take $D^{\bs}(\br, \bx^{\bs}) = \mathcal{I}^{2 \times 2}$. To achieve a clustering of local $\bmu$-isolines close to $\partial \Omega$, the value of $a_i(\br)$ grows steeply in the vicinity of $\partial \hOmr$. As $\hOm$ is polygonal with straight-sided edges, it is most convenient to construct the $a_i(\bxi)$ in $\hOm$ and defining the $a_i(\br)$ through a push-forward into $\hOmr$. For this, we can utilise the canonical distance function \smash{$d_j^i(\bxi)$} to the boundary edge $L_j$ associated with patch $\hOm_i$ (we assume that each boundary patch is only associated with one boundary edge for convenience). If $\hOmr$ is the unit disc, such a distance function can also be defined in $\hOmr$ directly. Taking $a_i(\br) \gg 1$ close to the boundary furthermore urges local $\br(\bmu)$ isolines to slide only in the direction of \smash{$\widehat{\partial}_{\mu^{\perp}} \br$} such that the angle between $\partial \Omega$ and transverse isolines of $\bx^{\bs}(\bmu)$ is unchanged with respect to the solution for $D^{\bs} = \mathcal{I}^{2 \times 2}$. \\
% To tune the density of clustering, the distance function \smash{$d^i_j(\bxi)$} is composed with a function that leads to decay when the distance $d^i_j$ grows. A proficient choice is
% \begin{align}
% \label{eq:boundary_layer_ai_unscaled}
%     a_i(\bxi) = A_i \exp\left(-\mu (d^i_j(\bxi))^2 \right), \quad \text{where } \mu > 0 \text{ tunes the decay rate, while } A_i \gg 1.
% \end{align}
% If $a_i(\br)$ decays to essentially zero toward the facet $\br(\gamma_{ik})$ opposite to $\br(L_j)$, the diffusivity is nearly continuous across the interface between boundary patch $\br(\hOm_i)$ and interior patch $\br(\hOm_k)$ and no stabilisation on the patch vertices is required in practice. We are considering the geometry with reference parameterisation from Figure \ref{fig:throwing_star_reference_param}. Figure \ref{fig:throwing_star_domain_ai_unscaled} shows the associated parametric domain along with the collection of $a_i(\bxi)$ plotted on each individual boundary patch. Here, we take $\hOmr = \hOm$ such that $\br(\bxi) = \bxi$.
% \begin{figure}[h!]
% \centering
% \begin{subfigure}[c]{0.4 \textwidth}
%     \includegraphics[width=\textwidth, valign=c]{img/control/boundary_layers/throwing_star_param_ai_unscaled.png}
%     \caption{The parametric domain $\hOm$ showing the collection of the $a_i(\bxi)$ on each individual boundary patch.}
%     \label{fig:throwing_star_domain_ai_unscaled}
% \end{subfigure}
% \hspace*{1cm}
% \begin{subfigure}[c]{0.4 \textwidth}
%     \includegraphics[width=\textwidth, valign=c]{img/control/boundary_layers/throwing_star_ref.png}
%     \caption{A reference parameterisation for a geometry for which we would like to create a boundary layer.}
%     \label{fig:throwing_star_reference_param}
% \end{subfigure}
% \caption{The parametric domain $\hOm$ showing the collection of the $a_i(\bxi)$ on each patch along with a reference parameterisation of $\Om$}
% \label{fig:throwing_star_reference}
% \end{figure}
% Figure \ref{fig:throwing_star_unscaled} shows the resulting maps for the choices $A_i = 25$ and $A_i = 50$.
% \begin{figure}[h!]
% \centering
% \begin{subfigure}[c]{0.4 \textwidth}
%     \includegraphics[width=\textwidth, valign=c]{img/control/boundary_layers/throwing_star_unscaled_25.png}
%     \caption{The result of recomputing the map from Figure \ref{fig:throwing_star_reference_param} under~\eqref{eq:boundary_layer_ai_unscaled} with $A_i = 25$.}
%     \label{fig:throwing_star_unscaled_25}
% \end{subfigure}
% \hspace*{1cm}
% \begin{subfigure}[c]{0.4 \textwidth}
%     \includegraphics[width=\textwidth, valign=c]{img/control/boundary_layers/throwing_star_unscaled_50.png}
%     \caption{The result of recomputing the map with $A_i = 50$.}
%     \label{fig:throwing_star_unscaled_50}
% \end{subfigure}
% \caption{Figure showing the boundary layers created by~\eqref{eq:boundary_layer_ai_unscaled} with $A_i = 25$ and $A_i = 50$.}
% \label{fig:throwing_star_unscaled}
% \end{figure}
% The figure shows the creation of a boundary layer, which becomes more pronounced for $A_i = 50$. However, the layer creation is somewhat inhomogeneous and less pronounced in the protruding parts of the boundary. This is not surprising given that the local $\bmu$-isolines are significantly farther apart in these regions for the reference parrameterisation $\bx_h^{\br}: \hOm \rightarrow \Om$ from Figure \ref{fig:throwing_star_reference_param}. This can be addressed by introducing position-dependent amplitudes, i.e, $A_i \rightarrow A_i(\bxi)$. Given the averaged value of $\| \partial_{\mu^{\perp}} \bx_h^{\br} \|_{L^2(\partial \hOm)}$ i.e.,
% $$\overline{\| \partial_{\mu^{\perp}} \bx_h^{\br} \|} := \frac{\sqrt{\int_{\partial \hOm} \| \partial_{\mu^{\perp}} \bx_h^{\br}\|^2 \mathrm{d} \Gamma}}{\int_{\partial \hOm} \mathrm{d} \Gamma},$$
% we define $A_i(\bxi)$ on $L_j = \partial \hOm \cap \partial \hOm_i$ as
% $$A_i (\bxi) \vert_{L_j} = A \left(\frac{\partial_{\mu^{\perp}} \bx_h^{\br}(\bxi) \vert_{L_j}}{\overline{\| \partial_{\mu^{\perp}} \bx_h^{\br} \|}} \right)^k, \quad \text{for some } k > 0 \text{ and } A > 0.$$
% $A_i(\bxi) \vert_{\partial \hOm}$ is then extended into the interior of patch $\hOm_i$ by requiring $\partial_{\mu^{\perp}} A_i(\bxi) = 0$, where, as before, $\partial_{\mu^{\perp}}(\, \cdot \,)$ denotes the local directional derivative transversal to the boundary edge $L_j$ associated with boundary patch $\hOm_i$. The Euler-Lagrange equation associated with this choice of $D^{\bs}$ suggests that for $k = 2$, the value of $\|\partial_{\mu^{\perp}} \bx_h^{\bs}(\bx) \|$ can be expected to remain largely constant along $\partial \Omega$, which becomes the default choice.
% \begin{figure}[h!]
% \centering
% \begin{subfigure}[c]{0.4 \textwidth}
%     \includegraphics[width=\textwidth, valign=c]{img/control/boundary_layers/throwing_star_unscaled_50.png}
%     \caption{The result of recomputing the map from Figure \ref{fig:throwing_star_reference_param} under~\eqref{eq:boundary_layer_ai_unscaled} with $A_i = 25$.}
%     \label{fig:throwing_star_scaled_25}
% \end{subfigure}
% \hspace*{1cm}
% \begin{subfigure}[c]{0.4 \textwidth}
%     \includegraphics[width=\textwidth, valign=c]{img/control/boundary_layers/throwing_star_scaled_50.png}
%     \caption{The result of recomputing the map with $A_i = 50$.}
%     \label{fig:throwing_star_scaled_50}
% \end{subfigure}
% \caption{Figure showing the boundary layers created by~\eqref{eq:boundary_layer_ai_unscaled} with $A_i = 25$ and $A_i = 50$.}
% \label{fig:throwing_star_scaled}
% \end{figure}

==> sec-domain_optimization.tex <==
\section{Domain Optimization}
\label{sect:Adaptive_Domain_Optimization}
As demonstrated in Section \ref{subsect:Adaptive_Results}, the approach from Section \ref{sect:Adaptive_Basic_Scheme} can handle challenging geometries. However, it lacks the flexibility of precisely controlling the parametric properties of the outcome, which may lead to undesirable features, such as large elements (see Figures \ref{fig:solution_strategies} and \ref{fig:solution_strategies_ref}). As such, in the following we present a framework that allows for more flexibility, where we pay particular attention to mitigating the aforementioned pathologies associated with inversely harmonic maps. \\
Instead of mapping inversely harmonically into a domain $\hat{\Omega}$ with a Cartesian coordinate system, we now define it through a parameterization $\mathbf{s}: \hat{\Omega} \rightarrow \hat{\Omega}$. For convenience, we assume that the boundary correspondence $\mathbf{s} \vert_{\partial \hat{\Omega}}: \partial \hat{\Omega} \rightarrow \partial \hat{\Omega}$ is the identity. Suppose that $\mathbf{x}^*: \hat{\Omega} \rightarrow \Omega$ solves the equation
\begin{align}
    \Delta_{\mathbf{x}} \boldsymbol{\xi} = \mathbf{0}, \quad \text{s.t.} \quad \mathbf{x} \vert_{\partial \hat{\Omega}} = \mathbf{x}_D(\boldsymbol{\xi}),
\end{align}
for $\mathbf{x}$. Then, if $\mathbf{x}(\boldsymbol{\xi})$ is the solution of
\begin{align}
\label{eq:Adaptive_Strong_Equations_reparameterized}
    \Delta_{\mathbf{x}} \mathbf{s}(\boldsymbol{\xi}) = \mathbf{0}, \quad \text{s.t.} \quad \mathbf{x} \vert_{\partial \hat{\Omega}} = \mathbf{x}_D(\mathbf{s}(\boldsymbol{\xi})),
\end{align}
it clearly satisfies $\mathbf{x} = \mathbf{x}^* \circ \mathbf{s}$, thanks to the fact that $\mathbf{x}_D \circ \mathbf{s} = \mathbf{x}_D$ on $\partial \hat{\Omega}$ (i.e., the boundary condition does not change upon pullback). As such, we may approximate compositions $\mathbf{x}^* \circ \mathbf{s}$ by solving the discretized counterpart of (\ref{eq:Adaptive_Strong_Equations_reparameterized}). \\
Introducing the set of vectors
\begin{align}
    \mathbf{p}^{ij}(\mathbf{s}) = -T^{-1} \frac{\partial^2 \mathbf{s}}{\partial \boldsymbol{\xi}_i \partial \boldsymbol{\xi}_j}, \quad \text{with} \quad T = \partial_{\boldsymbol{\xi}} \mathbf{s} \quad \text{and} \quad (i, j) \in \{1, 2\} \times \{1, 2 \},
\end{align}
it can be shown that with $\mathbf{s} = \mathbf{s}(\boldsymbol{\xi})$, (\ref{eq:Adaptive_Strong_Equations_reparameterized}) can be reformulated as \cite[Chapter 4]{thompson1998handbook}
\begin{align}
A(\mathbf{x}) \colon \left( H(\mathbf{x}_i) + P^1(\mathbf{s}) \frac{\partial \mathbf{x}_i}{\partial \xi} + P^2(\mathbf{s}) \frac{\partial \mathbf{x}_i}{\partial \eta} \right) = 0 \quad i \in \{1, 2\}, \quad \text{s.t.} \quad \mathbf{x} \vert_{\partial \hat{\Omega}} = \mathbf{x}_D \vert_{\partial \hat{\Omega}}.
\end{align}
Here, the matrices $P^1$ and $P^2$ satisfy
\begin{align}
\label{eq:Adaptive_Control_matrices}
    P^k_{ij}(\mathbf{s}) = \mathbf{p}_{k}^{ij}(\mathbf{s}), \quad k \in \{ 1, 2 \}.
\end{align}
Therefore, we introduce
\begin{align}
\label{eq:Adaptive_F_operator_reparameterized}
    F(\mathbf{x}, \boldsymbol{\sigma}, \mathbf{s}) = \sum_{i=1}^2 \int_{\hat{\Omega}} \boldsymbol{\tau}( \boldsymbol{\sigma}, \mathbf{x})_i A(\mathbf{x}) : \underbrace{\left( H(\mathbf{x}_i) + P^1(\mathbf{s}) \frac{\partial \mathbf{x}_i}{\partial \xi} + P^2(\mathbf{s}) \frac{\partial \mathbf{x}_i}{\partial \eta} \right) \det T(\mathbf{s})}_{\tilde{H}(\mathbf{x}_i, \mathbf{s})} \mathrm{d}S,
\end{align}
and for given $\mathbf{s}(\boldsymbol{\xi})$, we solve
\begin{align}
\label{eq:Adaptive_inverse_mapping_approach_PDE_scaled_discretized_reparameterized}
    & \text{find } \mathbf{x}_h \in \mathcal{U}^{\mathbf{x}_D}_h \quad \text{s.t.} \quad F(\mathbf{x}_h, \boldsymbol{\sigma}_h, \mathbf{s})= 0 \quad \forall \boldsymbol{\sigma}_h \in \mathcal{U}^{\mathbf{0}}_h,
\end{align}
in order to approximate $\mathbf{x}^* \circ \mathbf{s}$. Unless stated otherwise, we utilize the Newton approach from Section \ref{subsect:Adaptive_Newton} with $\boldsymbol{\tau}(\boldsymbol{\sigma}, \mathbf{x}) = \boldsymbol{\sigma}$. We can apply the Picard approach from Section \ref{subsect:Adaptive_Picard} by replacing $H(\mathbf{x}_i) \rightarrow \tilde{H}(\mathbf{x}_i, \mathbf{s})$ in equation (\ref{eq:Adaptive_Picard_G_tau}). In the following, we present several strategies for choosing $\mathbf{s}$ to improve the parametric properties of the composite mapping.


\subsection{Exploiting the Maximum Principle}
\label{sect:Adaptive_Eploiting_Maximum_Principle}
Clearly, for well-posedness of (\ref{eq:Adaptive_inverse_mapping_approach_PDE_scaled_discretized_reparameterized}), $\mathbf{s}: \hat{\Omega} \rightarrow \hat{\Omega}$ should not fold. As the control mapping maps into a convex domain, we may exploit the fact that if it is the solution to a second order elliptic problem in divergence form, it is necessarily a bijection \cite{bauman2001univalent}. Thus, let $\mathbf{s} = (\mathbf{s}_1, \mathbf{s}_2)^T$ be such that
\begin{align}
\label{eq:Adaptive_forward_laplace_control_mapping}
    \nabla_{\boldsymbol{\xi}} \cdot \left(D \nabla_{\boldsymbol{\xi}} \mathbf{s}_i \right) = 0 \quad i \in \{1, 2\}, \quad \text{in} \quad \hat{\Omega}, \quad \text{s.t.} \quad \mathbf{s}(\boldsymbol{\xi}) = \boldsymbol{\xi} \text{ on } \partial \hat{\Omega},
\end{align}
where $D: \hat{\Omega} \rightarrow \mathbb{R}^{2 \times 2}$ is an SPD diffusivity tensor. In the following, we assume that an accurate approximation $\mathbf{x}^*_h$ of $\mathbf{x}^*$ has been computed using the methodology from Section \ref{sect:Adaptive_Basic_Scheme}. In order to mitigate the impact of the well-known pathologies of inversely harmonic maps (see Section \ref{sect:Adaptive_Solution_Strategies}), we may select $D$ in (\ref{eq:Adaptive_forward_laplace_control_mapping}) such that the value of
\begin{align}
\label{eq:Adaptive_L_Area}
    L_{\text{Area}}(\mathbf{x}_h) = \int_{\hat{\Omega}} \det J(\mathbf{x}_h)^2 \mathrm{d} S
\end{align}
is expected to decrease with respect to $\mathbf{x}^*$ (see (\ref{eq:Adaptive_Area_costfunc})). Note that
\begin{align}
\label{eq:Adaptive_Poisson_Area_equation}
    \left( \det J (\mathbf{x}^* \circ \mathbf{s}) \right)^2 & \simeq \left( \det \partial_{\mathbf{s}} \mathbf{x}_h^* \right)^2 \det J(\mathbf{s})^2 \nonumber \\
    & = \left( \det \partial_{\mathbf{s}} \mathbf{x}_h^* \right)^2 \left( g_{11} g_{22} - g_{12}^2 \right)_{\boldsymbol{\xi} \rightarrow \mathbf{s}} \nonumber \\
    & \leq \frac{1}{2} \left( \det \partial_{\mathbf{s}} \mathbf{x}_h^* \right)^2 \left( g_{11} + g_{22} \right)^2_{\boldsymbol{\xi} \rightarrow \mathbf{s}},
\end{align}
where the subscript $\boldsymbol{\xi} \rightarrow \mathbf{s}$ indicates that the $g_{ij}$ between brackets refer to the metric induced by $\mathbf{s}(\boldsymbol{\xi})$. Given that $\mathbf{s}(\boldsymbol{\xi}) = \boldsymbol{\xi}$ initially, (\ref{eq:Adaptive_Poisson_Area_equation}) suggests a convex optimization problem of the form
\begin{align}
\label{eq:Adaptive_PoissonArea_minimization}
    L_\text{PoissonArea}(\mathbf{s}, k) \rightarrow \min \limits_{\mathbf{s} \in \mathcal{V}_h^2}, \quad \text{s.t.} \quad \mathbf{s}(\boldsymbol{\xi}) = \boldsymbol{\xi}\text{ on } \partial \hat{\Omega},
\end{align}
where
\begin{align}
\label{eq:Adaptive_PoissonArea_costfunc}
    L_\text{PoissonArea}(\mathbf{s}, k) = \int_{\hat{\Omega}} \left( \det \partial_{\boldsymbol{\xi}} \mathbf{x}_h^* \right)^{k} \left( \| \partial_{\boldsymbol{\xi}} \mathbf{s}_1 \|^2 + \| \partial_{\boldsymbol{\xi}} \mathbf{s}_2 \|^2 \right) \mathrm{d}S,
\end{align}
for recomputing $\mathbf{s}(\boldsymbol{\xi})$. As such, we are solving the discretized equations corresponding to (\ref{eq:Adaptive_forward_laplace_control_mapping}) with
\begin{align}
\label{eq:Adaptive_Diffusivity_Area}
D = \left( \det \partial_{\boldsymbol{\xi}} \mathbf{x}_h^* \right)^{k} I^{2 \times 2}.
\end{align}
Even though the exact solution of (\ref{eq:Adaptive_forward_laplace_control_mapping}) does not fold, the discretized counterpart may fold due to extreme diffusive anisotropy. This can be counteracted by reducing the value of $k$. Alternatively, (\ref{eq:Adaptive_PoissonArea_costfunc}) can be utilized for DWR-based a posteriori refinement to achieve bijectivity and accuracy of $\mathbf{s}: \hat{\Omega} \rightarrow \hat{\Omega}$. \\
Upon completion, we compute $\mathbf{x}_h \in \mathcal{V}_h^2$ using the control mapping $\mathbf{s}: \hat{\Omega} \rightarrow \hat{\Omega}$, with a posteriori refinement if necessary.
\begin{figure}[h!]
  \centering
  \subfloat[]{\includegraphics[width=.45\linewidth]{img/chapter4/PoissonAreaPuzzle/k_0.png}\label{fig:PoissonAreaPuzzle_k_0}} \quad
  \centering
  \subfloat[]{\includegraphics[width=.45\linewidth]{img/chapter4/PoissonAreaPuzzle/k_05.png}\label{fig:PoissonAreaPuzzle_k_05}} \\
  \centering
  \subfloat[]{\includegraphics[width=.45\linewidth]{img/chapter4/PoissonAreaPuzzle/k_1.png}\label{fig:PoissonAreaPuzzle_k_1}} \quad
  \centering
  \subfloat[]{\includegraphics[width=.45\linewidth]{img/chapter4/PoissonAreaPuzzle/k_15.png}\label{fig:PoissonAreaPuzzle_k_15}}
  \centering
  \caption{Several parameterizations of the puzzle piece with reparameterization based on (\ref{eq:Adaptive_forward_laplace_control_mapping}) and (\ref{eq:Adaptive_Diffusivity_Area}) with the reference parameterization $k=0$ (a), reparameterization with $k=0.5$ (b), $k=1$ (c) and $k=1.5$ (d). }
  \label{fig:PoissonAreaPuzzle}
\end{figure}

\begin{figure}[h!]
  \centering
  \subfloat[]{\includegraphics[align=c, width=.45\linewidth]{img/chapter4/PoissonAreaPuzzle/detJ_PoissonArea_normal.png}\label{fig:PoissonAreaPuzzle_ReparameterizedDomain_normal}} \quad
  \centering
  \subfloat[]{\includegraphics[align=c, width=.45\linewidth]{img/chapter4/PoissonAreaPuzzle/detJ_PoissonArea.png}\label{fig:PoissonAreaPuzzle_ReparameterizedDomain_ReparameterizedDomain}}
  \caption{Plots showing the reference domain (a) and the reparameterized domain based on (\ref{eq:Adaptive_forward_laplace_control_mapping}) and (\ref{eq:Adaptive_Diffusivity_Area}) with $k=1.5$ (b). The figure clearly shows that the elements are contracted wherever $\det \partial_{\boldsymbol{\xi}} \mathbf{x}_h^*$ is large.}
  \label{fig:PoissonAreaPuzzle_ReparameterizedDomain}
\end{figure}

\begin{table}[h!]
\centering
\begin{tabular}{c|c|c|c|c}
$k$   & $0$ & $0.5$ & $1$ & $1.5$ \\ \hline
$L_\text{Area}(\mathbf{x}_h) \times 10^{-2}$ & $3.291$ & $2.077$ & $1.439$ & $1.299$
\end{tabular}
\captionsetup{justification=centering}
\caption{Evaluation of $L_\text{Area}(\mathbf{x}_h)$ for various values of k.}
\label{tab:L_PoissonArea_Puzzle_Piece}
\end{table}
\noindent Figure \ref{fig:PoissonAreaPuzzle} shows puzzle piece geometry parameterizations for various values of $k$, while Table \ref{tab:L_PoissonArea_Puzzle_Piece} contains the outcomes of substituting into (\ref{eq:Adaptive_L_Area}). Both clearly demonstrate that the methodology has the desired effect, with more drastic outcomes for larger values of $k$. Figure \ref{fig:PoissonAreaPuzzle_ReparameterizedDomain} shows the isolines of $\mathbf{s}(\boldsymbol{\xi})$ before and after reparameterization with $k=1.5$. All parameterizations were computed with the reference basis corresponding to Figure \ref{fig:PoissonAreaPuzzle_k_0}. No a posteriori refinements were necessary.

\begin{figure}[h!]
  \centering
  \subfloat[]{\includegraphics[align=c, width=.30\linewidth]{img/chapter4/indiana/Indiana_k_0.png}\label{fig:PoissonAreaIndiana_k_0}}
  \centering
  \subfloat[]{\includegraphics[align=c, width=.30\linewidth]{img/chapter4/indiana/Indiana_k_1.png}\label{fig:PoissonAreaIndiana_k_1}} \qquad
  \centering
  \subfloat[]{\includegraphics[align=c, width=.30\linewidth]{img/chapter4/indiana/Indiana_domain_k_1.png}\label{fig:PoissonAreaIndiana_k_1_domain}}
  \caption{Parameterization of the U.S. state of Indiana with $k=0$ (a), $k=1$ (b) and the corresponding reparameterized domain (c). }
  \label{fig:PoissonAreaIndiana}
\end{figure}
Figure \ref{fig:PoissonAreaIndiana} shows parameterizations of the U.S. state of Indiana for $k=0$ and $k=1$. Contrary to Table \ref{tab:L_PoissonArea_Puzzle_Piece}, with
\begin{align*}
    L_\text{Area}(\mathbf{x}_h) = 1.049 \times 10^2 \quad \text{for} \quad k=0 \quad \text{and} \quad L_\text{Area}(\mathbf{x}_h) = 1.008 \times 10^2 \quad \text{for} \quad k=1,
\end{align*}
the effect is very mild. Restricting the integrals to $\eta < 1/7$, however, the difference becomes more pronounced with
\begin{align*}
    L_\text{Area}(\mathbf{x}_h) = 17.167 \quad \text{and} \quad L_\text{Area}(\mathbf{x}_h) = 14.118,
\end{align*}
respectively. Unsurprisingly from the shape of the geometry, the difference is most striking close to the lower boundary, which can also be seen in the figure. A posteriori refinement was necessary in Figure \ref{fig:PoissonAreaIndiana_k_1}. \\
Heuristically, reparameterization based on the maximum principle proves to be one of the most robust and effective choices for a wide range of geometries while being computationally efficient. This is thanks to the fact that it addresses the known pathologies of inversely harmonic maps, while also yielding smooth solutions, which preserves smoothness of the composite mapping.

%%
\subsection{Constrained Domain Optimization}
The concept of reparameterizing the domain in order to alter the parametric properties of the recomputed geometry parameterization can be further extended in a way more reminiscent of the well-known cost function minimization approach (see Section \ref{sect:Adaptive_Introduction}). Given an accurate approximation $\mathbf{x}^*_h$ of $\mathbf{x}^*$ (see Section \ref{sect:Adaptive_Eploiting_Maximum_Principle}), we define the metric $G_{\mathbf{s} \rightarrow \mathbf{x}} = \partial_{\mathbf{s}} \mathbf{x}^T \partial_{\mathbf{s}} \mathbf{x}$, which is initially given by 
\begin{align*}
    G_{\mathbf{s} \rightarrow \mathbf{x}} = \partial_{\boldsymbol{\xi}} \mathbf{x}^{*T} \partial_{\boldsymbol{\xi}} \mathbf{x}^{*} \simeq \partial_{\boldsymbol{\xi}} \mathbf{x}^{*T}_h \partial_{\boldsymbol{\xi}} \mathbf{x}^{*}_h.
\end{align*}
Hence, in order to optimize $\mathbf{x}_h(\boldsymbol{\xi})$, we optimize $\mathbf{s}(\boldsymbol{\xi})$ in the metric induced by $G_{\mathbf{s} \rightarrow \mathbf{x}}$. With
\begin{align}
    g_{ij}^\mathbf{s} = \left[\partial_{\boldsymbol{\xi}} \mathbf{s}^T G_{\mathbf{s} \rightarrow \mathbf{x}} \partial_{\boldsymbol{\xi}} \mathbf{s} \right]_{ij} \quad \text{and} \quad J_{ij}^\mathbf{s} = [\partial_{\boldsymbol{\xi}} \mathbf{x}_h^* \partial_{\boldsymbol{\xi}} \mathbf{s}]_{ij},
\end{align}
we define domain optimization cost functions $Q_i^\mathbf{s}(\mathbf{s})$ by replacing $g_{ij} \rightarrow g_{ij}^{\mathbf{s}}$ and $J_{ij} \rightarrow J_{ij}^\mathbf{s}$ in the $Q_i$ introduced in equation (\ref{eq:Adaptive_weighted_sum}) (see Section \ref{sect:Adaptive_Introduction}). We may nevertheless choose to add terms of the form $Q_j(\mathbf{s})$, which should then be regarded as regularization terms. Let $\mathcal{U}_h^\square = \{ \mathbf{v} \in \mathcal{V}_h^2 \enskip \vert \enskip \mathbf{v} = \boldsymbol{\xi} \text{ on } \partial \hat{\Omega} \}$. A domain optimization problem takes the form
\begin{align}
\label{eq:Adaptive_Domain_Optimization_Problem}
    \int_{\hat{\Omega}} Q(\mathbf{s}) \mathrm{d}S \rightarrow \min \limits_{\mathbf{s} \in \mathcal{U}_h^\square}, \quad \text{s.t.} \quad \mathbf{C}(\mathbf{s}) \geq \mathbf{0},
\end{align}
with
\begin{align}
\label{eq:Adaptive_Domain_Q}
    Q(\mathbf{s}) = \sum_i \lambda_i^{\mathbf{s}} Q_i^{\mathbf{s}}(\mathbf{s}) + \sum_j \lambda_j Q_j(\mathbf{s}).
\end{align}
Here, the constraint $\mathbf{C}(\mathbf{s}) \geq 0$ ensures that the minimizer of (\ref{eq:Adaptive_Domain_Optimization_Problem}) does not fold. In the following, we list all choices of $\mathbf{C}(\mathbf{s})$ that come to mind. \\
Given the element segmentation $\mathcal{T}$ of $\hat{\Omega}$, by $\mathcal{V}^{p, \alpha}(\mathcal{T})$ we denote the canonical THB-space with order $p$ and regularity $\alpha$ that is compatible with $\mathcal{T}$. Note that $\alpha \leq p - 1$. Clearly, if $\mathcal{V}_h$ has order $p$ and regularity $\alpha \leq p-1$, this implies that 
\begin{align*}
    \det \partial_{\boldsymbol{\xi}} \mathbf{s} \in \mathcal{V}^{2p -1, \alpha-1}(\mathcal{T}).
\end{align*}
As such, we also have 
\begin{align*}
    \det \partial_{\boldsymbol{\xi}} \mathbf{s} \in \mathcal{V}^{2p-1, -1}(\mathcal{T}).
\end{align*}
Hence, we can base the constraint on B\'ezier extraction, in which we require that all weights of projecting $\det \partial_{\boldsymbol{\xi}} \mathbf{s}$ onto $\mathcal{V}^{2p-1, -1}(\mathcal{T})$ be positive. Let $\mathbf{\hat{d}}$ be the corresponding vector of weights. We have
\begin{align}
\label{eq:Adaptive_Bezier_Constraint}
    \mathbf{\hat{d}}(\mathbf{s}) = \hat{M}^{-1} \mathbf{\hat{f}}(\mathbf{s}) > \mathbf{0}, \quad \text{where} \quad \mathbf{\hat{f}}_i(\mathbf{s}) = \int \limits_{\hat{\Omega}} \hat{\phi}_i \det \partial_{\boldsymbol{\xi}} \mathbf{s} \mathrm{d}S,
\end{align}
with
\begin{align}
\hat{\phi}_i \in \left[ \mathcal{V}^{2p-1, -1}(\mathcal{T}) \right] \quad \text{and} \quad \hat{M}_{i,j} = \int \limits_{\hat{\Omega}} \hat{\phi}_i \hat{\phi}_j \mathrm{d}S.
\end{align}
Note that $\hat{M}$ is block-diagonal with $\vert \mathcal{T} \vert$ blocks of size $(2p, 2p)$. Hence, we computationally efficiently assemble $\hat{M}^{-1}$ simply by computing the inverse of all separate blocks leading to a sparse block-diagonal matrix. As such, the computational costs of testing whether the condition $\mathbf{\hat{d}} > \mathbf{0}$ is fulfilled reduces to the assembly of $\mathbf{\hat{f}}$ along with one sparse matrix-vector multiplication. Assembly of the constraint gradient of $\mathbf{\hat{d}}(\mathbf{c}_{\mathcal{I}})$, where $\mathbf{c}_{\mathcal{I}}$ is a vector containing the inner control points of $\mathbf{s}$, requires the assembly of $\partial_{\mathbf{c}_{\mathcal{I}}} \mathbf{\hat{f}}$ and a sparse matrix-matrix multiplication. The assembly is hence feasible. However, for large values of $p$ this may lead to an infeasibly large number of constraints. \\
Inspired by \cite{gravesen2012planar}, we formulate an alternative constraint by projecting $\det \partial_{\boldsymbol{\xi}} \mathbf{s}$ onto the coarser THB-space $\mathcal{V}^{2p-1, \alpha-1}(\mathcal{T})$. Similar to (\ref{eq:Adaptive_Bezier_Constraint}), this leads to a constraint of the form
\begin{align}
\label{eq:Adaptive_Gravesen_Constraint}
    \mathbf{d}(\mathbf{s}) = M^{-1} \mathbf{f}(\mathbf{s}) > \mathbf{0}, \quad \text{where} \quad \mathbf{f}_i(\mathbf{s}) = \int \limits_{\hat{\Omega}} \phi_i \det \partial_{\boldsymbol{\xi}} \mathbf{s} \mathrm{d}S, \end{align}
with
\begin{align}
\phi_i \in \left[ \mathcal{V}^{2p-1, \alpha - 1}(\mathcal{T}) \right] \quad \text{and} \quad M_{i,j} = \int \limits_{\hat{\Omega}} \phi_i \phi_j \mathrm{d}S.
\end{align}
Increasing the values of $p$ and $\alpha$, unlike for (\ref{eq:Adaptive_Bezier_Constraint}), the length of $\mathbf{d}$ in (\ref{eq:Adaptive_Gravesen_Constraint}) increases only slowly (thanks to $K$-refinement). On the other hand, the matrix $M$ is not block-diagonal and neither is it separable (unlike in a structured spline setting). As such, the assembly of the constraint gradient is prohibitively expensive. Here, a remedy is to introduce the vector of slack variables $\mathbf{e} > 0$. The constraint from (\ref{eq:Adaptive_Gravesen_Constraint}) can be reformulated as follows:
\begin{align}
    C_{\alpha}(\mathbf{s}, \mathbf{e}) = \mathbf{f}(\mathbf{s}) - M \mathbf{e} = \mathbf{0}, \quad \text{with} \quad \mathbf{e} > \mathbf{0}. 
\end{align}
Hence, we avoid inversion with $M$ at the expense of introducing an additional inequality constraint and changing the existing inequality constraint to an equality constraint. Note that we have:
\begin{align}
    \frac{\partial C_{\alpha}(\mathbf{s}, \mathbf{e})}{\partial (\mathbf{c}_{\mathcal{I}}, \mathbf{e})} = \left[ \frac{\partial \mathbf{f}}{\partial \mathbf{c}_{\mathcal{I}}}, -M \right] \quad \text{and} \quad \frac{\partial \mathbf{e}}{\partial (\mathbf{c}_{\mathcal{I}}, \mathbf{e})} = \left[ 0, I \right],
\end{align}
where $I$ denotes the identity matrix of appropriate dimension. 
\begin{figure}[h!]
\centering
  \subfloat[Depiction of the cones associated with the linear constraint $\mathbf{C}_L(\mathbf{x}_h)$ generated from the control net of a structured spline mapping for a bat-shaped geometry. The constraint is violated (the two associated cones intersect) despite the bijectivity of the mapping, demonstrating the restrictiveness of $\mathbf{C}_L(\mathbf{x}_h)$.]{\includegraphics[align=c, width=.9\linewidth]{img/chapter4/constraint/bat.png}\label{fig:linear_constraint_bat}} \\
  \subfloat[Control net of the Cartesian parametric domain. In this case, both cones collapse into half rays generated by $\mathbb{R}^+(1, 0)^T$ and $\mathbb{R}^+(0, 1)^T$, respectively. The feasible space may then be comprised of all parameterizations of $\hat{\Omega}$ with cones contained within $-\pi/4 < \theta < \pi/4$ and $\pi/4 < \theta < 3\pi/4$, respectively. Hereby, the initial guess is located exactly in the center of the feasible space.]{\includegraphics[align=c, width=.9\linewidth]{img/chapter4/constraint/domain.png}\label{fig:linear_constraint_domain}}
  \caption{Depiction of the bijectivity constraint $\mathbf{C}_L$ for a generic geometry (a), and the initially Cartesian parametric domain (b).}
  \label{fig:linear_constraint}
\end{figure}

% \begin{figure}[h!]
% \centering
%   \subfloat[]{\includegraphics[align=c, width=.3\linewidth]{img/chapter4/constrained_domain_detJ_puzzle/domain_refined_reparameterized.png}\label{fig:Puzzle_detJ_domain_refined_reparameterized}} $\qquad$
%   \subfloat[]{\includegraphics[align=c, width=.5\linewidth]{img/chapter4/constrained_domain_detJ_puzzle/puzzle_piece_optimized.png}\label{fig:Puzzle_detJ_geometry}}
%   \subfloat[]{\includegraphics[align=c, width=.3\linewidth]{img/chapter4/constrained_domain_detJ_regularized_puzzle/domain_reparameterized_refined.png}\label{fig:Puzzle_detJ_domain_refined_reparameterized_regularized}} $\qquad$
%   \subfloat[]{\includegraphics[align=c, width=.5\linewidth]{img/chapter4/constrained_domain_detJ_regularized_puzzle/puzzle_piece_optimized.png}\label{fig:Puzzle_detJ_geometry_regularized}}
%   \caption{Result of reparameterizing $\mathbf{s}(\boldsymbol{\xi})$ with $Q = Q^{\mathbf{s}}_{\text{Area}}$ (a) and the corresponding recomputed geometry parameterization (b). Figures (c) and (d) show the results of repeating these steps with an additional regularization term.}
%   \label{fig:Puzzle_detJ}
% \end{figure}

\begin{figure}[h!]
\centering
  \subfloat[]{\includegraphics[align=c, width=.45\linewidth]{img/chapter4/bezier_domain_AO_Indiana/Indiana_AO_bezier_domain.png}\label{fig:Indiana_AO_domain_reparameterized}} $\qquad$
  \subfloat[]{\includegraphics[align=c, width=.4\linewidth]{img/chapter4/bezier_domain_AO_Indiana/Indiana_AO_bezier.png}\label{fig:Indiana_AO_geometry}}
  \caption{Result of reparameterizing the domain corresponding to the U.S. state of Indiana with $Q = Q_{\text{AreaOrthogonality}}^{\mathbf{s}}$ (a) and the resulting recomputed geometry parameterization (b).}
  \label{fig:Indiana_AO}
\end{figure}

\noindent Given a set of abscissae $\boldsymbol{\Xi} = \{\boldsymbol{\xi}_1^c, \ldots \boldsymbol{\xi}_m^c \} \subset \mathbb{R}^2$, an alternative constraint $\mathbf{C}^{\boldsymbol{\Xi}}(\mathbf{s})$ follows from requiring that
\begin{align}
\label{eq:Adaptive_detJ_discrete_necessary}
    \boldsymbol{\epsilon}_i^L \leq \det \partial_{\boldsymbol{\xi}} \mathbf{s} (\boldsymbol{\xi}_i^c) \leq \boldsymbol{\epsilon}_i^U, \quad \forall i \in \{1, \ldots, m\},
\end{align}
where $\mathbb{R}^m \ni \boldsymbol{\epsilon}^{L, U} \geq 0$ are lower and upper thresholds. Note that (\ref{eq:Adaptive_detJ_discrete_necessary}) is nonlinear and nonconvex but not a sufficient condition for bijectivity of $\mathbf{s}$. However, it makes bijectivity likely for $m$ sufficiently large. \\
Finally, assuming that $\mathbf{s}$ is built from a structured basis $\left[ \mathcal{V}_h \right]$ resulting from a tensor product of the univariate bases
\begin{align*}
    \{ N_1^\square, \ldots, N_n^\square \} \quad \text{and} \quad \{ M_1^\square, \ldots, M_m^\square \},
\end{align*}
we may alternatively utilize the linear constraint proposed in \cite{xu2011parameterization}. Typically, we take $\left[ \mathcal{V}_h \right]$ as the cardinality-wise largest structured basis compatible with $\mathcal{T}$. Given
\begin{align}
    \mathbf{s}(\xi, \eta) = \sum_{i,j} \mathbf{c}_{i, j} N_i^\square(\xi) M_j^\square(\eta),
\end{align}
let the cones $\mathcal{C}^1(\mathbf{s})$ and $\mathcal{C}^2(\mathbf{s})$ be generated by the half rays $\mathbb{R}^+ \Delta_{i,j}^1$ and $\mathbb{R}^+ \Delta_{i, j}^2$ with
\begin{align*}
    \Delta_{i, j}^1 = \mathbf{c}_{i+1, j} - \mathbf{c}_{i, j} \quad \text{and} \quad \Delta_{i, j}^2 = \mathbf{c}_{i, j+1} - \mathbf{c}_{i, j},
\end{align*}
respectively. The constraint is based on the observation that if $\mathcal{C}^1(\mathbf{s})$ and $\mathcal{C}^2(\mathbf{s})$ only intersect in $\boldsymbol{\xi} = \mathbf{0}$, then $\mathbf{s}$ is bijective. In a direct optimization of $\mathbf{x}_h$, above constraint may be impractical since for most $\mathbf{x}_D$, the set 
\begin{align*}
\left \{ \mathbf{x}_h \in \mathcal{U}^{\mathbf{x}_D}_h \enskip \vert \enskip \mathcal{C}^1(\mathbf{x}_h) \cap \mathcal{C}^2(\mathbf{x}_h) = \{ \mathbf{0}\} \right \}
\end{align*}
is empty or the constraint is too restrictive. However, in the case of optimizing $\mathbf{s}$, for $\mathbf{s}^0 = \boldsymbol{\xi}$, the cones $\mathcal{C}^1(\mathbf{s}^0)$ and $\mathcal{C}^2(\mathbf{s}^0)$ are generated by $\mathbb{R}^+(1, 0)^T$ and $\mathbb{R}^+ (0, 1)^T$, respectively. A linear constraint $\mathbf{C}_L(\mathbf{s})$ follows from requiring that $\mathcal{C}^1(\mathbf{s})$ and $\mathcal{C}^2(\mathbf{s})$ be contained in the cones generated by 
\begin{align*}
     \mathbb{R}^+ \times \left \{(1, -1 + \epsilon)^T, (1, 1 + \epsilon)^T \right \} \quad \text{and} \quad  \mathbb{R}^+ \times \left \{(1, 1 + \epsilon)^T, (-1, 1 + \epsilon)^T \right \},
\end{align*}
respectively. Here $\epsilon \ll 1$ is a small positive parameter. Clearly, $\mathbf{s}^0$ is located exactly in the center of the feasible region (see Figure \ref{fig:linear_constraint}), making the constraint much less restrictive at the expense of having to compute $\mathbf{x}_h^*$ first.
\begin{remark}
We can combine the proposed constraints with the principles from Section \ref{sect:Adaptive_Eploiting_Maximum_Principle} to suppress overshoots due to extreme diffusive anisotropy. If $\mathbf{C}(\mathbf{s}) = \mathbf{C}_L(\mathbf{s})$, the problem remains convex.
\end{remark}
\noindent Figure \ref{fig:Indiana_AO_domain_reparameterized} shows the domain corresponding to the U.S. state of Indiana (see Figure \ref{fig:Indiana}) after optimizing with 
\begin{align*}
    Q = Q_{\text{AreaOrthogonality}}^{\mathbf{s}}
\end{align*}
under the constraint $\mathbf{C}(\mathbf{s}) = \hat{\mathbf{d}}(\mathbf{s})$ (see equation (\ref{eq:Adaptive_Bezier_Constraint})). The domain mapping $\mathbf{s}(\boldsymbol{\xi})$ is built from the same THB-basis as $\mathbf{x}^*_h$, comprised of $2338$ DOFs. Since Newton failed to converge, we recomputed $\mathbf{x}_h$ using the Picard approach, which converged after $21$ iterations. The result is depicted in Figure \ref{fig:Indiana_AO}. No a posteriori refinements were required. The reparameterization reduces the value of $L_{\text{AreaOrthogonality}}$ from the initial
\begin{align*}
L_{\text{AreaOrthogonality}}(\mathbf{x}_h^*) = 1.77 \times 10^2, \quad \text{to} \quad L_{\text{AreaOrthogonality}}(\mathbf{x}_h) = 1.36 \times 10^2.
\end{align*}
Next, we optimize the domain corresponding to the puzzle piece geometry (see Figure \ref{fig:solution_strategies_id}) with $\mathbf{C}(\mathbf{s}) = \mathbf{C}_L(\mathbf{s})$ and $Q = Q_{\text{Area}}^{\mathbf{s}}$. Hereby, $\mathbf{s}(\boldsymbol{\xi})$ is built from a structured spline space comprised of $646$ DOFs. The reparameterized domain is depicted in Figure \ref{fig:Puzzle_detJ_domain_linear_refined_reparameterized}.
\begin{figure}[h!]
\centering
  \subfloat[]{\includegraphics[align=c, width=.3\linewidth]{img/chapter4/constrained_domain_detJ_linear_constraint_puzzle/domain_reparameterized.png}\label{fig:Puzzle_detJ_domain_linear_refined_reparameterized}} $\qquad$
  \subfloat[]{\includegraphics[align=c, width=.5\linewidth]{img/chapter4/constrained_domain_detJ_linear_constraint_puzzle/puzzle_piece_optimized.png}\label{fig:Puzzle_detJ_linear_geometry}}
  \caption{Result of optimizing the puzzle piece domain with $Q = Q_{\text{Area}}^{\mathbf{s}}$ under the constraint $\mathbf{C}(\mathbf{s}) = \mathbf{C}_L(\mathbf{s})$ (a) and the corresponding recomputed mapping (b).}
  \label{fig:Puzzle_detJ_linear}
\end{figure}
Bijectivity of $\mathbf{x}_h$ is achieved with $2632$ DOFs and the resulting parameterization is depicted in Figure \ref{fig:Puzzle_detJ_linear_geometry}. With $L_\text{Area}(\mathbf{x}_h) = 142.710$, it is roughly as effective as the reparameterization from Figure \ref{fig:PoissonAreaPuzzle} with $k = 1$. \\
Figure \ref{fig:NRW_orth_linear} shows the German province of North Rhine-Westphalia upon reparameterization with 
\begin{align*}
Q = Q_\text{Orthogonality}^\mathbf{s},
\end{align*}
where $\mathbf{s}(\boldsymbol{\xi})$ is built from a structured spline space comprised of $578$ DOFs, with $\mathbf{C}(\mathbf{s}) = \mathbf{C}_L(\mathbf{s})$. Initially, \begin{align*}
    L_{\text{Orthogonality}}(\mathbf{x}_h^*) = 18.929, \quad \text{while} \quad L_{\text{Orthogonality}}(\mathbf{x}_h) = 5.160
\end{align*}
upon recomputation. Bijectivity is achieved with $4584$ DOFs, which is roughly double the initial $2724$ DOFs.
\begin{figure}[h!]
\centering
  \subfloat[]{\includegraphics[align=c, width=.3\linewidth]{img/chapter4/NRW_orth_linear/domain_reparameterized_refined.png}\label{fig:NRW_orth_domain_refined_reparamterized}} $\qquad$
  \subfloat[]{\includegraphics[align=c, width=.5\linewidth]{img/chapter4/NRW_orth_linear/NRW_optimized.png}\label{fig:NRW_orth_linear_geometry}}
  \caption{Result of reparameterizing the reference parameterization of the German province of North Rhine-Westphalia (see Figure \ref{fig:NRW}), with $Q(\mathbf{s}) = Q_{\text{Orthogonality}}^{\mathbf{s}}(\mathbf{s})$. The reparameterized domain is shown in (a), while (b) shows the recomputed parameterization.}
  \label{fig:NRW_orth_linear}
\end{figure}

\begin{figure}[h!]
\centering
  \subfloat[]{\includegraphics[align=c, width=.3\linewidth]{img/chapter4/NRW_AO_linear/domain_reparameterized_refined.png}\label{fig:NRW_AO_domain_refined_reparamterized}} $\qquad$
  \subfloat[]{\includegraphics[align=c, width=.5\linewidth]{img/chapter4/NRW_AO_linear/NRW_optimized.png}\label{fig:NRW_AO_linear_geometry}}
  \caption{Result of reparameterizing the reference parameterization of the German province of North Rhine-Westphalia (see Figure \ref{fig:NRW}), with $Q(\mathbf{s}) = Q_{\text{AreaOrthogonality}}^{\mathbf{s}}(\mathbf{s})$. The reparameterized domain is shown in (a), while (b) shows the recomputed parameterization.}
  \label{fig:NRW_AO_linear}
\end{figure}
Finally, Figure \ref{fig:NRW_AO_linear} shows the result of reparameterizing the same geometry with 
\begin{align*}
Q = Q^{\mathbf{s}}_\text{AreaOrthogonality}
\end{align*}
and the same constraints. Initially, 
\begin{align*}
    L_{\text{AreaOrthogonality}}(\mathbf{x}_h^*) = 51.244, \quad \text{while} \quad L_{\text{AreaOrthogonality}}(\mathbf{x}_h) = 30.896
\end{align*}
upon recomputation. Bijectivity is achieved with only $2928$ DOFs.

\subsection{Direct Optimization}
As an alternative to operating in the parametric domain, we may choose to directly optimize the geometry parameterization with respect to a quality cost function. As an advantage, we avoid the (possibly expensive) recomputation of $\mathbf{x}_h$. In order to avoid folding, constraints should be employed. As a disadvantage, the linear constraint $\mathbf{C}_L(\mathbf{x}_h)$ cannot be used and the initial guess $\mathbf{x}^{*}_h$ may fail to satisfy the conditions $\mathbf{\hat{d}}(\mathbf{x}_h) > \mathbf{0}$ (cf. (\ref{eq:Adaptive_Bezier_Constraint})) and $\mathbf{d}(\mathbf{x}_h) > \mathbf{0}$ (cf. (\ref{eq:Adaptive_Gravesen_Constraint})) despite being bijective. Heuristically, for complicated geometries, this is usually the case. In such cases, the only viable constraint is $\mathbf{C}^{\Xi}(\mathbf{x}_h)$ (cf. (\ref{eq:Adaptive_detJ_discrete_necessary})). \\
We optimize the puzzle piece geometry with $Q(\mathbf{x}_h) = Q_{\text{Area}}(\mathbf{x}_h)$ under the constraint $\mathbf{\hat{d}}(\mathbf{x}_h) > 0$, where the initial guess $\mathbf{x}_h^{*}$ is the parameterization from Figure \ref{fig:PoissonAreaPuzzle_k_0}.
\begin{figure}[h!]
\centering
  \subfloat[]{\includegraphics[align=c, width=.3\linewidth]{img/chapter4/direct/puzzle_piece_Area_domain.png}\label{fig:puzzle_piece_Area_direct_domain}} $\qquad$
  \subfloat[]{\includegraphics[align=c, width=.5\linewidth]{img/chapter4/direct/puzzle_piece_Area_optimized.png}\label{fig:puzzle_piece_Area_direct_geometry}}
  \caption{The puzzle piece geometry after $21$ iterations of minimizing $Q(\mathbf{x}_h) = Q_{\text{Area}}$ under the constraint $\mathbf{\hat{d}}(\mathbf{x}_h) > 0$ (b) and the corresponding domain (a). The minimization was initialized with the parameterization from Figure \ref{fig:PoissonAreaPuzzle_k_0}.}
  \label{fig:puzzle_piece_Area_direct_30}
\end{figure}
Figure \ref{fig:puzzle_piece_Area_direct_30} shows the resulting parameterization. Convergence is achieved after $21$ constrained iterations. The reparameterization reduces $L_{\text{Area}}$ from the initial $L_{\text{Area}}(\mathbf{x}_h^*) = 3.29 \times 10^2$ to $L_{\text{Area}}(\mathbf{x}_h) = 0.96 \times 10^2$, which is slightly more pronounced than the reduction from Figure \ref{fig:PoissonAreaPuzzle} with $k=1.5$. However, the resulting parameterization is less regular compared to Figure \ref{fig:PoissonAreaPuzzle_k_15}, which can be remedied by adding a regularization of the form $Q(\mathbf{x}_h) = Q_{\text{Area}}(\mathbf{x}_h) + \beta Q_{\text{Uniformity}}(\mathbf{x}_h)$.
\begin{figure}[h!]
\centering
  \subfloat[]{\includegraphics[align=c, width=.4\linewidth]{img/chapter4/direct/Indiana_Area_40_domain.png}\label{fig:Indiana_Area_direct_domain}} $\qquad$
  \subfloat[]{\includegraphics[align=c, width=.4\linewidth]{img/chapter4/direct/Indiana_Area_40_optimized.png}\label{fig:Indiana_Area_direct_geometry}}
  \caption{The parameterization of the U.S. state of Indiana after $30$ iterations of minimizing $Q(\mathbf{x}_h) = Q_{\text{Area}}$ (b) and the corresponding domain (a). The minimization was initialized with the parameterization from Figure \ref{fig:PoissonAreaIndiana_k_0}.}
  \label{fig:Indiana_Area_direct_40}
\end{figure}
Next, we optimize the U.S. state of Indiana with $Q(\mathbf{x}_h) = Q_{\text{Area}}(\mathbf{x}_h)$ under the constraint $\mathbf{C}^{\boldsymbol{\Xi}}(\mathbf{x}_h) \geq 0$ with
\begin{align}
\label{eq:Adaptive_Lower_Upper_puzzle_direct_orth}
    \boldsymbol{\epsilon}_i^L  = \alpha_L \times \det J(\mathbf{x}_h^*)(\boldsymbol{\xi}_i^c) \quad \text{and} \quad \boldsymbol{\epsilon}_i^U  = \alpha_U \times \det J(\mathbf{x}_h^*)(\boldsymbol{\xi}_i^c),
\end{align}
(see equation (\ref{eq:Adaptive_detJ_discrete_necessary})). \\
Figure \ref{fig:Indiana_Area_direct_40} shows the resulting parameterization after $30$ iterations. With 
\begin{align*}
    L_{\text{Area}}(\mathbf{x}_h^*) = 1.049 \times 10^2 \quad \text{and} \quad L_{\text{Area}}(\mathbf{x}_h) = 0.989 \times 10^2,
\end{align*}
the reduction is mild, yet somewhat more pronounced than in Figure \ref{fig:PoissonAreaIndiana}. Here, $\boldsymbol{\Xi}$ results from uniform sampling with $36$ points per element. The choice of the relaxation factors $0 \leq \alpha_L \leq 1$ and $1 \leq \alpha_U$ in (\ref{eq:Adaptive_Lower_Upper_puzzle_direct_orth}) tunes to which degree trading an increase in $L_\text{Area}$ for a decrease in the employed cost function is acceptable. Here, more conservative choices lead to less cost function reduction but to more uniform cell sizes and vice versa. Furthermore, values of $\alpha_L$ closer to $1$ prevent the grid from folding, even if fewer sampling points are used. We used $\alpha_L = 0.05$ and $\alpha_U = 4$.

\subsection{Achieving Boundary Orthogonality}
\begin{figure}[h!]
\centering
  \subfloat[]{\includegraphics[align=c, width=.4\linewidth]{img/chapter4/boundary_orth/sin_reference/domain_reference.png}\label{fig:sin_bndry_orth_reference_domain}} $\qquad$
  \subfloat[]{\includegraphics[align=c, width=.5\linewidth]{img/chapter4/boundary_orth/sin_reference/geometry_reference.png}\label{fig:sin_bndry_orth_reference_optimized}}
  \caption{Reference parameterization of a tube-like shaped geometry which is to be orthogonalized by the northern and southern boundaries.}
  \label{fig:sin_bndry_orth_reference}
\end{figure}
Many applications favor parameterizations with isolines that are orthogonal to the boundary contours. One way to achieve this is allowing $\lambda_i^{\mathbf{s}} = \lambda_i(\boldsymbol{\xi})^{\mathbf{s}}$ in (\ref{eq:Adaptive_Domain_Q}) and taking $\lambda_\text{Orthogonality}^{\mathbf{s}}$ large close to $\partial \hat{\Omega}$. We are considering the example of achieving orthogonality at the northern and southern boundaries of the geometry depicted in Figure \ref{fig:sin_bndry_orth_reference}. To this end, we minimize the cost function \begin{align*}
    Q(\mathbf{s}) = (1 + \lambda_{\text{O}}(\boldsymbol{\xi})) Q^{\mathbf{s}}_{\text{Orthogonality}},
\end{align*}
where $\lambda_{\text{O}}(\boldsymbol{\xi})$ takes on large values close to the northern and southern boundaries of $\partial \hat{\Omega}$. We employ the constraint $\mathbf{C}(\mathbf{s}) = \mathbf{C}_L(\mathbf{s})$, where $\mathbf{s}(\boldsymbol{\xi})$ is built from a structured spline space comprised of $594$ DOFs. The resulting parameterization is depicted in Figure \ref{fig:sin_bndry_orth}.
\begin{figure}[h!]
\centering
  \subfloat[]{\includegraphics[align=c, width=.4\linewidth]{img/chapter4/boundary_orth/sin_penalty/sin_domain_reparameterized.png}\label{fig:sin_bndry_orth_domain_refined_reparamterized}} $\qquad$
  \subfloat[]{\includegraphics[align=c, width=.5\linewidth]{img/chapter4/boundary_orth/sin_penalty/sin_optimized.png}\label{fig:sin_bndry_orth_optimized}}
  \caption{Result of reparameterizing the geometry mapping from Figure \ref{fig:sin_bndry_orth_reference} by weakly enforcing boundary orthogonality through a large penalty term (b) and the corresponding reparameterized domain (a).}
  \label{fig:sin_bndry_orth}
\end{figure}
The figure indeed shows a large degree of orthogonalization, which is somewhat weaker in the protruded parts of the geometry. This is due to orthogonality only being enforced \textit{weakly} through a penalty term. More pronounced boundary orthogonalization may be achieved by taking $\lambda_\text{O}$ larger close to $\partial \hat{\Omega}$. \\
Let $\gamma_e, \gamma_w, \gamma_s$ and $\gamma_n$ refer to the eastern, western, southern and northern parts of $\partial \hat{\Omega}$, respectively. For a more drastic boundary orthogonalization, we follow the approach from \cite[Chapter ~6]{thompson1998handbook}, which consists of solving the problem
\begin{align}
\label{eq:Adaptive_boundary_orth_laplace}
    \Delta_{\mathbf{x}^*_h} f = 0 \quad \text{s.t.} \quad f = 0 \text{ on } \gamma_e, \enskip f = 1 \text{ on } \gamma_w \quad \text{and} \quad \frac{\partial f}{\partial \mathbf{n}} = 0 \text{ on } \gamma_s \cup \gamma_n
\end{align}
on an initially folding-free geometry parameterization $\mathbf{x}_h^*$. Here, $\mathbf{n}$ denotes the unit outward normal vector on $\partial \Omega$. Upon completion, the control mapping $\mathbf{s} = (\mathbf{s}_1, \mathbf{s}_2)^T \equiv (s, t)^T$ is computed from
\begin{align}
\label{eq:Adaptive_control_mapping_boundary_orth_PDE}
    s(\xi, \eta) = f(\xi, 0) H_0(\eta) + f(\xi, 1) H_1(\eta) \quad \text{and} \quad t(\xi, \eta) = \eta,
\end{align}
where
\begin{align}
    H_0(\eta) = (1 + 2 \eta)(1 - \eta)^2 \quad \text{and} \quad H_1(\eta) = (3 - 2 \eta) \eta^2
\end{align}
are cubic Hermite interpolation functions. It can be shown that with this choice of $s$ and $t$, the solution of (\ref{eq:Adaptive_Strong_Equations_reparameterized}) is orthogonal at $\gamma_s$ and $\gamma_n$.  We approximately solve for $f$ by computing the solution $f_h$ of the discretized counterpart of (\ref{eq:Adaptive_boundary_orth_laplace}) over some structured spline space $\mathcal{V}_h$. Hereby, the Neumann boundary conditions are weakly imposed through partial integration. The control mapping follows from replacing $f \rightarrow f_h$ in (\ref{eq:Adaptive_control_mapping_boundary_orth_PDE}). Should orthogonality at $\gamma_w$ and $\gamma_e$ be desired, we simply exchange the roles of $s \rightarrow t$, $(\gamma_s, \gamma_n) \rightarrow (\gamma_w, \gamma_e)$ and $\xi \rightarrow \eta$.
\begin{remark}
Unlike $f$, $f_h$ may fail to be monotone increasing on $\gamma_s$ or $\gamma_n$, leading to a folded control mapping $\mathbf{s}(\boldsymbol{\xi})$.
\end{remark}
\begin{figure}[h!]
\centering
  \subfloat[]{\includegraphics[align=c, width=.4\linewidth]{img/chapter4/boundary_orth/sin_PDE/domain_reparameterized.png}\label{fig:sin_bndry_orth_PDE_domain_refined_reparamterized}} $\qquad$
  \subfloat[]{\includegraphics[align=c, width=.5\linewidth]{img/chapter4/boundary_orth/sin_PDE/geometry_optimized.png}\label{fig:sin_bndry_orth_PDE_optimized}}
  \caption{Result of reprameterizing the geometry mapping from Figure \ref{fig:sin_bndry_orth_reference} using the approach proposed in \cite[Chapter ~6]{thompson1998handbook} (b) and the corresponding reparameterized domain (a).}
  \label{fig:sin_bndry_orth_PDE}
\end{figure}
Figure \ref{fig:sin_bndry_orth_PDE} shows the recomputed parameterization of the same geometry using the preceding methodology, along with the reparameterized parametric domain, which has been computed from the same structured spline basis as in Figure (\ref{fig:sin_bndry_orth}). The figure shows an outstanding boundary orthogonalization, which comes at the expense of larger elements in the protruded parts compared to Figure \ref{fig:sin_bndry_orth}. We introduce another control mapping $\mathbf{s}^\prime(\boldsymbol{\xi})$, which we compute from the solution of
\begin{align}
\label{eq:Adaptive_minimization_s_prime_orth}
    \int_{\hat{\Omega}} (\det \partial_{\mathbf{s}} \mathbf{x}_h)^k (g_{11} + \beta g_{22})_{\mathbf{s} \rightarrow \mathbf{s}^\prime} \det \partial_{\boldsymbol{\xi}} \mathbf{s} \mathrm{d} S \rightarrow \min \limits_{\mathbf{s}^\prime \in \mathcal{V}_h^2}, \quad \text{s.t.} \quad \mathbf{s}^\prime(\boldsymbol{\xi}) = \mathbf{s}(\boldsymbol{\xi}) \text{ on } \partial \hat{\Omega},
\end{align}
where $\mathbf{s} = (s, t)^T$ and $\mathbf{x}_h$ correspond to Figures \ref{fig:sin_bndry_orth_PDE} (a) and (b), respectively. Here, the $g_{ii}$ correspond to diagonal entries of the metric tensor associated with the diffeomorphism between $\mathbf{s} \vert_{\hat{\Omega}}$ and $\mathbf{s}^\prime \vert_{\hat{\Omega}}$. As before, $k > 0$ tunes to which degree the spread in cell size is penalized, while $\beta > 1$ tunes the degree to which $\mathbf{s}^\prime$ is contracted / expanded in the direction of $\partial_{\eta} \mathbf{s}$, in order to compensate for large / small cells in $\mathbf{x}_h$. Taking $\beta$ large essentially freezes $\mathbf{s}^\prime$ in the direction of $\partial_{\xi} \mathbf{s}$, such that boundary orthogonality is preserved. Note that in (\ref{eq:Adaptive_minimization_s_prime_orth}), we are essentially solving the discrete counterpart of
\begin{align}
    \nabla_{\mathbf{s}} \cdot( D \nabla_\mathbf{s} \mathbf{s}^\prime_i ) = 0, \quad i \in \{1, 2\}, \quad \text{s.t.} \quad \mathbf{s}^\prime(\boldsymbol{\xi}) = \mathbf{s}(\boldsymbol{\xi}), \quad \text{with} \quad D = (\det \partial_{\mathbf{s}} \mathbf{x}_h)^k \begin{pmatrix} 1 & 0 \\ 0 & \beta \end{pmatrix}.
\end{align}
\begin{figure}[h!]
\centering
  \subfloat[]{\includegraphics[align=c, width=.4\linewidth]{img/chapter4/boundary_orth/sin_PDE_rep/domain_reparameterized.png}\label{fig:sin_bndry_orth_PDE_rep_domain_refined_reparamterized}} $\qquad$
  \subfloat[]{\includegraphics[align=c, width=.5\linewidth]{img/chapter4/boundary_orth/sin_PDE_rep/geometry_optimized.png}\label{fig:sin_bndry_orth_PDE__rep_optimized}}
  \caption{Result of reprameterizing the geometry mapping from Figure \ref{fig:sin_bndry_orth_PDE} using the principles from Section \ref{sect:Adaptive_Eploiting_Maximum_Principle} (b) and the corresponding reparameterized domain (a).}
  \label{fig:sin_bndry_orth_PDE_rep}
\end{figure}
Figure \ref{fig:sin_bndry_orth_PDE_rep} shows the geometry parameterization along with the reparameterized domain upon recomputation with $k = 0.75$ and $\beta = 300$. Compared to Figure \ref{fig:sin_bndry_orth_PDE}, the figure shows a much better cell size distribution, in particular close to the boundaries. Large cells can be further penalized by increasing the value of $k$.
%%
%\subsection{Heuristics}

==> sec-multiply_connected_domains.tex <==
\section{Multiply Connected Domains}

\subsection{Periodic domains}

\subsection{Punctured domains}

\subsection{General genus $N$ domains}
